On the Dynamics of Political Discussions on Instagram: A Network Perspective

Instagram has been increasingly used as a source of information especially among the youth. As a result, political figures now leverage the platform to spread opinions and political agenda. We here analyze online discussions on Instagram, notably in political topics, from a network perspective. Specifically, we investigate the emergence of communities of co-commenters, that is, groups of users who often interact by commenting on the same posts and may be driving the ongoing online discussions. In particular, we are interested in salient co-interactions, i.e., interactions of co-commenters that occur more often than expected by chance and under independent behavior. Unlike casual and accidental co-interactions which normally happen in large volumes, salient co-interactions are key elements driving the online discussions and, ultimately, the information dissemination. We base our study on the analysis of 10 weeks of data centered around major elections in Brazil and Italy, following both politicians and other celebrities. We extract and characterize the communities of co-commenters in terms of topological structure, properties of the discussions carried out by community members, and how some community properties, notably community membership and topics, evolve over time. We show that communities discussing political topics tend to be more engaged in the debate by writing longer comments, using more emojis, hashtags and negative words than in other subjects. Also, communities built around political discussions tend to be more dynamic, although top commenters remain active and preserve community membership over time. Moreover, we observe a great diversity in discussed topics over time: whereas some topics attract attention only momentarily, others, centered around more fundamental political discussions, remain consistently active over time.

==> 2_related_work_CARLOS.tex <==
\section{Related work}
\label{sec:related}

\begin{itemize}
    \item \textbf{We need to remove some related work very carefully. It got really big.}
\end{itemize}

We characterize political discussions on Instagram by analyzing user interactions from a network perspective. Three bodies of work are related to our effort: i) studies on online discussions in social media; ii) efforts to model interactions among groups of users (i.e., co-interactions); and iii) methods to extract network backbones.

%\subsection{User behavior and interactions on social media}

%The use of social media as a platform for political debate has already been studied. Twitter, in particular, has been analyzed in the context of political polarization~\cite{Vergeer:2015, Gorkovenko:2017, Nguyen:2018, Weaver:2019}, user engagement~\cite{Caetano:2018, kuvsen:2018, Badawy:2018} and politicians' behavior~\cite{Chi:2010}. Other works target Facebook~\cite{Tanase:2020, fabricio} and WhatsApp~\cite{Resende:2019, Josemar:2019}. Such types of analysis are however rare in the case of Instagram.

%Regarding Instagram, some studies focused on how different types of content or profiles engage users. Considering a broad (non-political) perspective, Kang et al.~\cite{Kang:2020} studied how a well-known strategy to trigger user interactions in social media affects discussions, namely mentioning friends in comments. Jaakonmäki et al.~\cite{Jaakonm:2017} analyzed the influence of posted content on social media marketing. Yang et al.~\cite{Yang:2019} studied brand mentioning practices of influencers. In contrast to those works, we focus on user behavior around political figures on Instagram.

%Closer to our work, Zarei et al.~\cite{Zarei:2019} analyzed user engagement around twelve Instagram profiles divided into different categories (e.g., sports, news and politics) searching for users who simulate others' behavior, e.g., to spread fake news.  Mu\~{n}oz et al.~\cite{Munoz:2017} studied image content posted by candidates during the US 2016 primary elections. Trevisan et al.~\cite{Trevisan:2019} performed a quantitative study of the political debate on Instagram, highlighting that politicians' profiles tend to attract more interactions than others. To the best of our knowledge, we are the first to analyze a network of co-commenters on Instagram and the emergence of communities around salient co-commenters. We complement those previous efforts by providing an orthogonal and broader analysis of the dynamics of communities who engage in political discussions.

\subsection{Online discussions in social media applications}

Several social media applications have been largely studied as platforms for political debate. For example, Nguyen ~\cite{Nguyen:2018}  presented a literature review of the role of Twitter on politics, notably as a platform to help politicians win elections and foster political polarization. Indeed, many studies have already argued for the increasing polarization in political orientation~\cite{Gruzd:2014, Vergeer:2015}, whereas others have explored the benefits that politicians can have from using Twitter to reach their supporters~\cite{Chi:2010}. 

Gorkovenko et al. studied user behavior on Twitter during live political debates, finding that people often use the platform to share their opinions, make provocative  statements, and inform others~\cite{Gorkovenko:2017}. Badawy et al.~\cite{Badawy:2018}, in turn,  found evidence of the use of Twitter for political manipulation. Caetano et al., in turn, analyzed the behavior of politically engaged user groups on Twitter during the 2016 US presidential campaign \cite{Caetano:2018}. Using information from user profiles, contact networks and tweet content, the authors identified four different groups, namely advocates for both main candidates, bots and regular users, and analyzed their behavior in terms of language patterns, popularity and how tweets from each candidate affected the mood expressed in their messages.  

Online discussions have also been studied in the context of other platforms. For example, Tasente \cite{Tanase:2020} studied the political debate around the \textit{Brexit} on Facebook, analyzing messages that generated higher engagement from users. In~\cite{fabricio}, the authors developed a system to detect political ads on Facebook and used it to present evidence of misuse during the Brazilian 2018 elections. 
In that direction, WhatsApp has also been the target of recent studies as an important platform for political debate and information dissemination, notably for the spread of fake news during political elections \cite{Resende:2019, Josemar:2019, Nobre:2020, Maros:2020}. 

Considering Instagram, in particular, the literature on user behavior and interactions is reasonably recent and somewhat restricted. Some authors have analyzed user engagement~\cite{Yang:2019, Kim:2020} and properties of the textual content shared by Instagram users~\cite{Zhan:2018, Arslan:2019}, but with no particular focus on political discussions. Closer to our present effort,  Zarei et al.~\cite{Zarei:2019} analyzed user engagement of twelve Instagram profiles, including profiles of politicians, searching for \emph{impersonators} -- i.e., users who simulate others' behavior to perform specific activities, such as spreading fake news.   Mu\~{n}oz et al.~\cite{Munoz:2017} studied image content posted  by candidates during the US 2016 primary elections, highlighting combined factors that attract user engagement, whereas Trevisan et al.~\cite{Trevisan:2019} performed a quantitative study of the political debate on Instagram, highlighting that politicians' profiles tend to have significantly more interactions than others. 


Moreover, other studies have also analyzed user engagement on online discussions from different perspectives on Instagram. For example, Kang et al.~\cite{Kang:2020} studied a well-known strategy to trigger user interactions in social media, namely mentioning a friend in a comment. The authors proposed a model capable of classifying mentions into three categories based on its motivation:  information-oriented,  relationship-oriented, and  discussion-oriented. 
Jaakonmäki et al.~\cite{Jaakonm:2017} analyzed the influence of the content posted for social media marketing. They used machine learning algorithms to extract textual and visual content features from  posts, along with creator and context features, to  model their influence on user engagement. 
In another direction, Yang et al.~\cite{Yang:2019} studied the brand mentioning practices of influencers, finding that audience has highly similar reactions to sponsored and non-sponsored posts. They also proposed a neural network model to classify the sponsorship of posts combining network embedding  with features related to the posts and followers. Similarly, 
Kim et al. \cite{Kim:2020} proposed a multimodal deep learning model that uses contextual information of posts, including textual and image content,  to classify influencers as well as their posts into specific topics, such as food, fashion and traveling. 

In contrast to prior studies, we here take a completely different perspective by analyzing online discussions on Instagram, notably discussions on political subjects, through the less of a co-interactions network.  In particular, we focus on discussions triggered by posts of particular influencers. As such, co-interactions occur among users who comment on the same post. To the best of our knowledge, we are the first to analyze political discussions on Instagram from a network perspective. Indeed, the case study we address here largely complements prior studies of user interactions around political subjects \cite{Zarei:2019, Munoz:2017, Trevisan:2019} by offering a much broader analysis of the dynamics of communities
of users who engage in political discussions. Our present effort builds on a preliminary work~\cite{Ferreira:2020} where we focused on identifying the structure emerging from the co-commenter network, offering a novel methodology for backbone extraction in this kind of network.  We here greatly extend our prior effort by offering a much more thorough characterization of the content and temporal properties of communities extracted from this backbone.



\subsection{Modeling interactions among groups of users}

\textbf{CUIDADO: para nao cortar os trabalhos que os revisores sugeriram... }
\textbf{Idilio, agora que me toquei... Temos que colocar alguns trabalhos dessa seção na anterior, pq é online discussion. O problema é tbm é analizado do ponto de vista de co-interação, co-retweet, co-link sharing... Como fazemos com isso?}

A plethora of phenomena related to human interactions online and in the real world have been analyzed using concepts from complex networks. Yet, many of these interactions occur among multiple (potentially two or more) entities simultaneously, here referred to as  \textit{co-interactions}. The modeling of co-interactions has been explored across different frontiers. For example, the adoption of models based on time series has allowed studies on how the preference for content generated by influential users favors bursts of engagement on Twitter \cite{De:2020}. In \cite{Mitra:2017}, the authors showed a relationship between the dynamics of news spreading on Twitter and their level of credibility. They observed that news with lower levels of credibility tends to attract more users to spread them. Lehmann et al. \cite{Lehmann:2012} showed that the diffusion of hashtags on Twitter analyzed from a collective perspective is naturally driven by exogenous factors. That is, co-interactions through hashtags posts are mostly expressed by common feelings that instigate users' actions. Popularity of online content \cite{Lu:2019-co-drive, Lu:2020, De:2020}, human mobility \cite{Silva:2017, Yang:2016},  market transaction \cite{Peron:2011, Mateo:2019, Saeedian:2019} are other notable examples where co-interactions has been studied. 

Focusing on network-oriented models, closer to the goals of this work, a number of studies target the analysis the co-interactions notably in social media applications. For example, Lu et al. \cite{Lu:2020} proposed a framework for modeling  cascading social systems (e.g., Twitter and Weibo). The authors found that users following the same profile can be organized into different groups, each one with particular characteristics driving such co-interactions, e.g., timing, structure, posts topic, and user interests. The author of \cite{Liu2018:collectiveFacebook} used the Facebook and Wiki-talk (A dataset build on edits on user talk pages on Wikipedia) aimed at understanding how user's  \textit{social signature} changes over time considering their ego network.  In the same direction, Xu et al.~\cite{Xu:2018} aimed at developing strategies to predict user behavior, given some knowledge of the behavior adopted by the user's neighbors in the network.

By associating users with common interests, Awal et al.~\cite{Awal:2019} examined collective preferences by adopting an overlapping community detection approach. Their goal was  to extract information and predict which categories of articles a user would read or would be interested in reading, based on his/her social collective actions on a consumer review site. Gao et al. modeled human behavior during different extreme events by correlating data from Twitter and GoogleTrends. The goal of the authors was to  assess how human risk and emotional intensity generate collective responses in different regions and how these responses evolve over time. The results of a case study of the  2011 Japanese earthquake show different communities emerging with different perceptions and actions about the event studied \cite{Gao:2016}. Similarly, Kuvsen et al.\cite{Kuvsen:2020} analyzed the communication pattern among groups of users on Twitter in the face of several natural disasters. The authors reveal how the discussions around the observed disasters exhibit a different underlying structure in terms of connectivity (motifs) varying according to the sentiment of messages. In a broader analysis, Zhao et al. \cite{Zhao:2010} examine how motifs representing distinct structures of communication in different Online Social Networks. 


Acknowledging the distinct properties of co-interactions, some recent studies have empirically analyzed them through the lens of \textit{higher-order} network models. Such models focus on preserving the different structures of connectivity that can occur as two or more individuals interact with each other \cite{Battiston:2020, Yoon:2020}. In the most basic form, these structures are represented by different motifs (e.g., triangular motifs, star, structural hubs, etc) \cite{Benson:2016b, Rossi:2018}. Indeed, Benson et al.~\cite{Benson:2016b} explored the diversity of such co-interactions to analyze how they build networks with diverse structural patterns. Similarly, Rossi et al.~\cite{Rossi:2018} proposed a general framework to learn higher-order structures embedding representations  based on distinct motifs, while others have used neural networks to extract latent patterns from signals to forecast new co-interactions  \cite{Meng:2018, Hu:2019}. Adamic et al.~\cite{Adamic:2008} analyzed how co-interactions take place on Yahoo Answers. The authors found differing kinds of interaction represented by motifs in the question-answer networks that vary according to the topic. 


Here, we focus on the densest and most uniform form of co-interactions, where all individuals interact with each other, a particular type of motif known as clique \cite{Battiston:2020}. For such case, the literature adopts different nomenclatures, including \textit{sets} of interactions, sequences of \textit{associations}, \textit{cliques}, and \textit{multi-actor} interactions \cite{Kumar:2019, Lerner:2019, Battiston:2020, Yoon:2020}. These co-interactions constitute an important substructure for some complex systems, exhibiting diverse properties that are relevant to the study of the (often global) phenomenon of interest \cite{Benson2:2018, Meng:2018}. Examples of such co-interactions are online shopping carts with a set of items being purchased together, co-authors of scientific publications, people co-visiting the same places driven by cultural interests, groups of users commenting or sharing the same topic on a social media application \cite{Yang:2016, Benson:2018, Newman:2018, Nobre:2020, Giglietto:2020, Brito:2020}. 

Moreover, we are interested in looking at how a sequence of such co-interactions, driven by actions of interest of multiple individuals build a network.  To that end, we model them by projecting them into a weighted and undirected graph where nodes (or vertices) correspond to individuals and a weighted edge links two individuals according if they have already interacted. The weight corresponds to the number of interactions both individuals shared in common during the period under analysis.  However, as already argued \cite{Liebig:2016, Benson:2018, Coscia:2019, Cao:2019,  Kumar:2020}, such projected networks may include a large number of random, sporadic and weak edges that are not really part of the fundamental underlying network component representing the target phenomenon. Indeed, although this practice of projecting the original network into a graph of pairwise connections has been widely adopted, little attention has been paid to understanding how the projection considering all co-interactions may obfuscate relevant structural properties in the projected network.

For example, Cruickshank et al. \cite{Cruickshank:2020} proposed to analyze interaction among topics on Twitter by modeling a sequence of networks of co-interaction built on co-occurrences of hashtags used by tweet users. Moreover, other information is considered to model the network, for instance, the textual similarity of Tweets using the same hashtag. Then, a community detection method is applied to identify topical clusters of hashtags. In another work, the authors analyzed the online hate of such communities \cite{Uyheng:2021}. Similarly, Pacheco et al. use different features (e.g., similar hashtags, images or chronological events) of users to model co-interactions between them. With that, the authors reveal different patterns that suggest coordinated behavior on Twitter.


More recently, some studies have shown the importance of removing random or weak edges to reveal an underlying structure (i.e., the backbone) in networks formed by co-interactions \cite{Grinberg:2019, Malang:2020, Coscia:2019, Mattsson:2020, Mattsson2:2020, Jaffe:2020, Jiang:2020}. For example, Leão et al. showed how removing random edges in co-authoring networks converge to a topology with more pure social relationships and better quality community structures, compared to the original complete network \cite{Leao2018}. Another example is the study of information dissemination on the WhatsApp platform \cite{Nobre:2020}, where the authors explored a network of co-sharing patterns (i.e., a network connecting users who shared the same piece of content) to reveal important properties of information spread on the platform. 

Similarly, Giglietto et al. \cite{Giglietto:2020} analyzed posts about the general Italian and European Parliament elections on Facebook focusing on identifying inauthentic behavior. By modeling link of co-sharing network, the authors analyzed the network for the dissemination include distinct entities (pages, groups, and verified public profiles) that share the same content frequently in a short period of time. To do it, the authors propose an approach to identify a list of entities that performed \textit{near-simultaneous link sharing}, thus focusing on the most important co-interactions. Other works propose to adopt a broader interaction definition, which considers, for example, users co-retweeting, using the same hashtags or URLs (co-URL), mentioning the same accounts, or joining the same 'conversation' when reply chains with a common root tweet at the same time \cite{Hanteer:2018, Weber:2020}. Focusing on understand patterns of interactions, they  adopt a thresholding approach to remove edges with a low frequency. 
Pacheco et al. \cite{Pacheco:2020} proposed a set of network models also focused on revealing coordinated behavior on Twitter. Each model capture  different patterns of co-interactions between users extracted from contextual information om the traces of user behavior. For instance, they model co-interaction network by considering use of similar hashtags, users sharing of the same images or chronological use of the platform. Also, they consider a threshold approach to filter out edges less representative.  %The results show that the networks were not only composed of political-oriented entities, but also by those that demonstrated themselves as places of entertainment, forming heterogeneous networks and with different standards. 


\textbf{Simplificar - Falar que nenhuma das abordagem consideram a natureza havy tail de OSNs -> Usuarios muito ativos e conteudos muito populares... } 

In short, there is a large number of studies using different models focused on modeling co-interactions. Similar to some of the aforementioned prior efforts, we here also propose a network-oriented approach.  Naturally, the collective actions of groups of individuals constitute what we here refer to as \textit{co-interactions}, which can be modeled by a network and favors the extraction of patterns of different natures (e.g., structural, contextual and temporal). Besides part of them propose to select the most important edges for your study \cite{Leao2018, Hanteer:2018, Weaver:2019, Pacheco:2020, Giglietto:2020, Nobre:2020}, the most neglect some aspects of paramount importance that we will discuss and address throughout this paper. In particular, many such co-interactions occur from random and sporadic behavior, thus reflecting very weak relations from the perspective of analyzing co-interactions to understand the target phenomenon.   Thus, it is important to filter out such noise,  focusing only on those network edges that are really relevant (or salient) for the purpose of the phenomenon  \cite{Benson2:2018, De:2020, Ghalmane:2020}. 

\textbf{Simplificar...}

Here, our main hypothesis is that considering these previously neglected elements together can provide valuable insights about the co-interactions in a given system. Thus, as part of our approach to study online discussion, we must tackle the challenges of using the projected network in a very rich but dynamic environment, notably the presence of a potentially large number of weak and possibly irrelevant edges in online social applications. Unlike of the prior works, we investigate strategies that remove such noise and reveal edges in our co-commenters network that, in fact, contribute to the study of information dissemination from the co-interaction of users on Instagram.  Moreover, we investigate strategies to extract the backbone in such context and discuss their limitations in the next section shedding light into a new approach for address such challenge.   


\subsection{Network backbone extraction}

Network models and algorithms rely on the basic assumption that edges connecting nodes in the network faithfully represent the interactions that drive the phenomenon under study. Yet, as already mentioned, there is an extensive debate on the consequences of ignoring data quality in such models since algorithms can be misled by the presence of noise in the network -- e.g., edges formed by random, sporadic, weak interactions or even by measurement errors \cite{Slater:2009, Rahimi:2015, Newman:2018, Kobayashi:2019}. To address this problem, backbone extraction methods try to remove such noise and uncover a clearer image of the fundamental structure governing the network. These algorithms take as input the original network and provide a reduced version composed of \textit{salient} edges, that is, edges that should more faithfully represent the phenomenon under study \cite{Coscia:2017}. 

In general, methods for extracting backbone can be classified as \textit{global} or \textit{local}. Global methods consider information from the entire network and apply a pre-defined general rule  (e.g., a \textit{threshold}) to all edges to define which edges should be kept in the network \cite{Grady:2012, Yan:2018}. On the other hand, local methods define a subspace in the network delimited by a subset of elements - either edges or nodes - and use information extracted from such subspace to determine whether or not an edge should remain in the network \cite{Serrano:2009, Coscia:2017}. In both cases, statistical criteria are commonly defined to assist in edge pruning.

One of the simplest and most intuitive global methods is based on setting a threshold for removing edges whose weights are smaller than a given value $\tau$. It has been widely used in several contexts, for example, online social networks \cite{Rahimi:2015} and network traffic analysis \cite{Soro:2020}. This approach is particularly adequate when the salient edges are to some extent defined by the problem context (e.g., the edges with heavier weights are of interest to the phenomenon under study), making the use of a threshold single, global threshold principled \cite{Yan:2018}. Otherwise, the use of thresholds raises some concerns. Indeed, some studies argue about potential misinterpretations of the results when using threshold-based approaches, as they could introduce biases in the analyses \cite{Tsur:2017}. For example, setting the threshold  adequately is context-dependent and, as such, may be quite complex. Sometimes it is even not clear whether the same threshold  should be applied to all edges \cite{Garrison:2015}.

Another global method was proposed in \cite{Grady:2012}. It extracts the network backbone through a sampling process which entails calculating the tree of shortest paths connecting the given node to all other nodes on the network. Then, the distribution of the number of times that an edge appears in these shortest paths is used to determine whether a given edge is salient. Note that if an edge was created at random but still plays an important structural role in the network, it's likely to be considered salient by this method. This approach has been adopted to studying on phenomena related to interactions between species (for biological purposes) \cite{Ma:2019}, investigating attacks from global terrorism networks \cite{Malang:2020}, and analyzing the properties of co-authorship networks from the perspective of influential nodes \cite{Petri:2013}.	

Rather than relying on a general criterion (a single threshold or a single probability distribution) to extract the backbone, other methods are based on local properties specific to a single edge/node or a subset of edges/nodes. For instance,  in \textit{the disparity filter} method proposed by Serrano et al. is based on the assumption that an edge is salient if two nodes are connected with a disproportionately high weight compared to the weights connecting them to their other neighbors. In other words, salient edges are those that have weights that deviate significantly from the null hypothesis that the weights of all edges incident to a given node are uniformly distributed. Thus, edges are expressed as parts of the total edge weights of a node. These parts are then compared to a reference model, and $p$-values are used to determine how much an edge differs from it. The $p$-values are then used to prune the non-salient edges \cite{Serrano:2009}.


Noise Corrected \cite{Coscia:2017} is also a local backbone extraction method that is based on the assumption that the salience of a given edge results from a collaboration between the nodes. Unlike the disparity filter, this method is able to preserve peripheral-peripheral connections by estimating the expectation and variance of edge weights using a  binomial distribution, while, at the same time,  considering the propensity of the origin node  and the destination node to emit and receive edges. Thus, to be regarded as  salient, an edge must exceed its expected weight considering the connection strength of both nodes. This method has been applied to prior studies on human mobility \cite{Coscia:2020-Nature} and  economic activity \cite{Mattsson:2020}.


A somewhat different local approach exploits the concept of neighborhood overlap \cite{Ghalmane:2020}, which reveals the tie strength between a pair of nodes in terms of the fraction of common neighbors. The intuition is that the network backbone should be composed only of ties (edges) with strength above a certain threshold. This approach has been applied to analyze collaborations in co-authorship networks \cite{Brandao:2017}, provide recommendations of places through the structure of the underlying network of contacts \cite{Valverde:2018}, and to address routing in a mobile ad-hoc network as a strategy to reach a reliable path among the various connections \cite{Gupta:2017}. 


Noise corrected and disparity filter are examples of methods that estimate the structure of the underlying network using a \textit{reference model}. In particular, these methods assume a reference model describing how the network should be built under certain assumptions -- e.g., interactions occur by chance, based on independent behavior or the weights of all edges incident to a node are normally distributed \cite{Jacobs:2015, Silva:2014}. This reference model guides the definition of an edge weight distribution or even a generative process of the network, under the predefined assumptions. This distribution (or generative process) is used to filter out edges, leaving only those that deviate enough (in a probabilistic sense) from the given assumptions. 

For example, under the assumption of independent behavior, the authors of \cite{Silva:2014} proposed to remove edges whose weights are below the $95^{th}$ percentile of the reference edge weight distribution. The intuition is that these edges may have been formed by pure chance under the assumption of independent behavior. In contrast, the remaining edges, whose weights are too large to be formed by independent behavior (i.e., with low probability - 5\%),  should represent interactions that are indeed relevant to the study and thus should be kept as part of the backbone. Alternatively, the authors of \cite{Leao2018} proposed to extract random edges by classifying the interactions of the nodes through a measure of \textit{strength}. Such \textit{strength} is calculated taking into account the neighborhood overlap metric and the interaction's regularity over a given period of time. Then, a random graph with the same properties of the observed graph (i.e., degree distribution, number of nodes, and edges) is built and the \textit{strength} of edges is also computed. Last, each edge in the observed graph is compared against the corresponding one in the built random graph so as to classify it as either random or social. 


Yet, another family of methods focuses on specific domains, trying to use contextual information to generate a domain-specific reference model. Examples include techniques developed to support the study of recommendation systems under online commercial networks~\cite{Zeng:2016}, urban mobility patterns~\cite{Manca:2017}, transportation networks~\cite{Wu:2006} and wireless sensor networks~\cite{Kumar:2020}. These prior efforts offer evidence that relying on contextual information to design reference models can significantly improve the backbone extraction task. In contrast to this, some authors have suggested taking temporal factors into account when extracting the network backbone -- e.g., considering a sequence of snapshots of the network. For example, Kobayashi et al.~\cite{Kobayashi:2019} proposed to extract the backbone by exploiting a reference model based on the activity level of users in a sequence of snapshots of the network.  Similarly, Nadini et al.~\cite{Nadini:2019} propose a model for detecting the network backbone by exploiting temporal patterns of node interactions. 

We here employ a generative model to extract the backbones from co-commenters networks. This method was originally proposed in a preliminary version of this work \cite{Ferreira:2019}.  In contrast to the aforementioned methods, our model considers the fundamental elements and structure of the target domain (influencers, commenters and posts). Specifically, it takes into account post popularity and user activity level as factors to model independent user behavior on a per-edge basis, keeping only edges that deviate significantly from it. As such, our method relies on a fine-grained local reference model to keep only salient edges, thus revealing the network backbone. 

==> 2_related_work_OLD.tex <==
\section{Related work}\label{sec:related}

Our focus is the characterization of the political discussion on Instagram, relying on concepts and models from complex networks as fundamental tools to drive a large part of our study. Thus, there are mainly four large bodies of work that closely relate to our investigation: i) studies about user behavior and interactions on Instagram, including efforts to analyze the system as platform for political debate; ii) analyses of political discussions in online social networks in general; iii) efforts to model many-to-many interactions (such as the co-commenter interactions we here analyze); and iv) methods to extract noisy edges from a network so as to reveal its underlying backbone. We review relevant prior work on  these four directions next.

\subsection{User interactions on Instagram}

The literature on user interactions on Instagram is reasonably recent and not yet rich. Some studies focused on how different types of content or profiles attract user engagement, notably in the political context. For example, Zarei et al.~\cite{Zarei:2019} analyzed user engagement of twelve Instagram profiles divided into different categories (namely, sports, news and politics), searching for \emph{impersonators} -- i.e., users who simulate others' behavior to perform specific activities, such as spreading fake news.   Mu\~{n}oz et al.~\cite{Munoz:2017} studied image content posted  by candidates during the US 2016 primary elections, highlighting combined factors that attract user engagement, whereas Trevisan et al.~\cite{Trevisan:2019} performed a quantitative study of the political debate on Instagram, highlighting that politicians' profiles tend to have significantly more interactions than others.
%The authors also found that users comment more and for longer periods about politics, with a large number of replies that are usually not explicitly requested.  

With no specific focus on political debates, other studies have also analyzed user engagement from different perspectives. For example, Kang et al.~\cite{Kang:2020} studied a well-known strategy to trigger user interactions in social media, namely mentioning a friend in a comment. The authors proposed a model capable of classifying mentions into three categories based on its motivation:  information-oriented,  relationship-oriented, and  discussion-oriented. 
Jaakonmäki et al.~\cite{Jaakonm:2017} analyzed the influence of the content posted for social media marketing. They used machine learning algorithms to extract textual and visual content features from  posts, along with creator and context features, to  model their influence on user engagement. 
In another direction, Yang et al.~\cite{Yang:2019} studied the brand mentioning practices of influencers, finding that audience has highly similar reactions to sponsored and non-sponsored posts. They also proposed a neural network model to classify the sponsorship of posts combining network embedding  with features related to the posts and followers. Similarly, 
Kim et al. \cite{Kim:2020} proposed a multimodal deep learning model that uses contextual information of posts, including textual and image content,  to classify influencers as well as their posts into specific topics, such as, food, fashion and traveling. 

Other studies have analyzed properties of the textual content shared by Instagram users. For example, Zhan et al.~\cite{Zhan:2018} analyzed the sentiment of captions of Instagram posts to provide a preview of the content to the reader. Arslan et al.~\cite{Arslan:2019} also used sentiment analysis tools to develop a message-level emotion  classifier, with the goal of detecting cyberbullying. With a similar goal, Gupta et al.~\cite{Gupta:2020} focused on the temporal perspective, showing that, cyberbullying activities exhibit recurrent temporal patterns such as the occurrence of bursts. In the same direction, Kao et al.~\cite{Kao:2019} proposed a social role detection framework  to analyze cyberbullying on online social platforms, taking Instagram as one of their case studies. The framework considers the roles of victim, bully and supporter, which are automatically identified by analyzing comment network and linguistic properties.

%Weerasinghe et al.~\cite{Weerasinghe:2020} studied the formation of an ecosystem composed by groups of users in Telegram with the aim of obtaining facilitate reciprocity abuse on Instagram posts, where each member reciprocally interacts with content posted by other members of the group. 


%Among various ways of interacting in online social networks,  cyberbulling has been gaining strength in recent years, often driven by hate speech. A number of recent studies have analyzed cyberbulling on Instagram, aiming at using sentiment analysis tools to build a message-level emotion automatic classifier \cite{Arlan:2019}, analyzing recurrent temporal patterns cite{Gupta:2020}

%Weerasinghe et al.~\cite{Weerasinghe:2020} studied the formation of an ecosystem composed by groups of users in Telegram with the aim of obtaining facilitate reciprocity abuse on Instagram posts, where each member reciprocally interacts with content posted by other members of the group. In the same direction, Kao et. al~\cite{Kao:2019} propose a framework to understand cyberbullying using Instagram as a case study. They propose a framework to identify the presence of victim, bully, and supporter automatically, and whether a user’s social roles and behaviors are consistent over time according to their behavior.

%Commonly associated with hate speech, cyberbullying on Instagram has been studied primarily through sentiment analysis tools as presented by Arslan et al.~\cite{Arslan:2019}. The authors address the problem of cyberbullying through a message-level emotion automatic classifier, able to predict emotion labels for each comment in a previously annotated dataset. Gupta et al.~\cite{Gupta:2020}, on the other hand, seeks to extend this analysis to the temporal perspective. Based on a supervised model, the authors show that, in fact, cyberbullying activities exhibit recurrent temporal patterns such as the occurrence of burst. Also, they highlight the importance of considering the temporal dimension in platform debates. In a more superficial way, Zhan et al.~\cite{Zhan:2018} propose to analyze the sentiment of post captions on Instagram in order to provide the reader a preview of the content that will can be found in the post.  %https://dl.acm.org/doi/pdf/10.1145/3341105.3373956


Our present effort is orthogonal to the aforementioned studies as it focuses on the {\it network} that emerges as users engage in online debates by commenting on the same posts, an aspect mostly neglected so far, especially in the political context. Indeed, our work largely complements prior studies of user interactions around political subjects \cite{Zarei:2019, Munoz:2017, Trevisan:2019} by offering a much broader analysis of the dynamics of communities of users who engage in political discussions. The emergence of such communities as well as some basic topological and temporal properties have been discussed in a preliminary version of this work~\cite{Ferreira:2020}. We here perform a deeper analysis, by delving into the textual properties of the discussions these communities engage in (including sentiment and psycholinguistic properties) as well as on the temporal dynamics of the main topics discussed. By doing so, we are able to offer a more comprehensive investigation on how political discussions take place on Instagram.

%In our preliminary version of this work \cite{Ferreira:2020} we analyze how the interaction among commenters emerges on the Instagram. We here extend that prior effort by extending our analysis on a dynamic perspective and delving into the content of interest to the communities. 


%We observed that these works focus on analyzing the behavior of users in Online Social Network, mainly, on Instagram from various perspectives and using different types of models. However, little attention has been devoted considering dynamic behaviors of Instagram' users compared to the range of static analysis proposed. In contrast to these works, we here focus on networks of co-commenters studying their structure and dynamic behaviors. We propose a generative model able to reveal the most significant interactions between users. After, we dive on the structural aspects of the networks from emerging structures on user interactions and characterize the behavior of users in the political debate from different perspectives, including sentiment of debate, textual and psycholinguist properties. Also, we explore aspects in two countries and in a varied scenario, analyzing a large number of users in a long time span.

\subsection{Political discussions on other social media platforms}

%The growing use of online social networks in recent years has attracted the attention of several researchers to analyze the behavior of users in these networks with various goal, thought different methodologies and considering several case studies \cite{Tang:2017}.

In contrast to Instagram, other social media applications have been largely studied from the perspective of platforms for political debate. Twitter, in particular, has been the target of a large number of studies. As a summary of prior efforts, Nguyen ~\cite{Nguyen:2018}  presented a literature review of the role of Twitter on politics, discussing prior findings in terms of the effectiveness of the platform to help politicians win elections,  political polarization, and who benefits from using Twitter in the political arena. 
Indeed, many studies have already argued for the increasing polarization in political orientation \cite{Gruzd:2014, Vergeer:2015}, whereas others have explored the benefits that politicians can have from using Twitter to reach their supporters. 
For example, Chi and Yang suggested that politicians can significantly benefit from using Twitter, as they are able to establish networks with their peers and acquire their support \cite{Chi:2010}. 


In \cite{Gorkovenko:2017}, the authors studied user behavior on Twitter during live political debates. They observed that people often use the social network to share their opinions, experiences, make provocative or humorous statements, and interact and inform others. In ~\cite{Caetano:2018}, the authors analyzed the behavior of politically engaged user groups on Twitter during the 2016 US presidential campaign. Using information from user profiles, contact networks and tweet content, the authors identified four different groups, namely advocates for both main candidates, bots and regular users, and analyzed their behavior in terms of language patterns, popularity and how tweets from each candidate affected the mood expressed in their messages. In \cite{Badawy:2018}, the authors found evidence of the use of Twitter for political manipulation.

The online debate has also been studied in the context of other social networks. For example, Tasente \cite{Tanase:2020} analyzed the political debate around the \textit{Brexit} on Facebook. The author focused on the frequency at which European institutions spoke about Brexit on their Facebook pages and on identifying and analyzing the messages that generated higher engagement from users. In ~\cite{fabricio}, the authors developed a system to detect political ads on Facebook and used it to present evidence of misuse during the Brazilian 2018 elections. In that direction, WhatsApp has also been the target of recent studies as an important platform for political debate and information dissemination, notably for the spread of fake news during political elections \cite{Resende:2019, Josemar:2019}. 

In contrast to prior studies, we here take a completely different perspective by analyzing the network of co-commenters on Instagram and the emergence of groups of discussion around particular influencers and topics. This network, similarly to other online social networks (e.g., network of reviewers on Reddit, \cite{Buntain:2014}, network of co-listening users on Spotify \cite{Raunak:2020}, network of co-sharing medias on WhatsApp \cite{Nobre:2020}), is characterized by many-to-many interactions, which, as argued in the previous sections, brings several challenges to the investigation. As such, a contribution of our work is the design of a method to filter out random and spurious edges that emerge in the network, thus revealing its underlying fundamental components. By doing so, our work greatly complements the existing knowledge by presenting a thorough investigation of political discussions on an emerging social network. 

%\id{Here we focus too much on the fact that we take the backbone. I would instead add something about findings, since other works also filter out noise when evaluating other OSNs.}


\subsection{Modeling many-to-many interactions}

A plethora of phenomena related to human interactions online and in the real world have been analyzed
using concepts from complex networks. Often, these phenomena are modeled as a set of pairwise interactions, leading up to a graph model composed by nodes and edges whose structural topology can be characterized with traditional metrics such as density, diameter, clustering coefficient and number of connected components, among others \cite{Easley:2010}. Yet, many of these interactions occur among multiple (potentially more than two) entities simultaneously, constituting an important substructure for some complex systems and exhibiting diverse properties \cite{Benson2:2018, Meng:2018}. Examples of such {\it many-to-many} interactions are: online shopping carts with a set of items being purchased together, co-authors in scientific publications, co-interactions among proteins, sets of tags referenced in forums, e-mails sent to a subgroup of people, deputies taking the stand to vote during a voting session and groups of users commenting on the same topic on a social network \cite{Benson:2018, Ferreira:2019, Newman:2018, Resende:2019}.

 
%You should add this reference \cite{Rossetti:2018} reference. It was been cited in an unrelated setnence. It is about communities.


%Complex networks constitute a set of theoretical and analytical tools to describe and analyze phenomena related to interactions occurring in the real world \cite{Rossetti:2018}. In recent years, most of the systems used by these models have been models through pairwise connections. However, many of these interactions occur between three or more entities simultaneously, constituting a crucial substrucutres for some complex systems and exhibiting diverse properties \cite{Benson2:2018, Meng:2018}. For example, online shopping carts with a set of items being purchased together, co-authors in scientific publications, co-interactions between proteins, tags referenced in forums, e-mails sent to a subgroup of people, deputies taking a stand to vote during a voting session, groups of users under a post on a social network whether commenting or sharing on social networks and instant messengers \cite{Benson:2018, Ferreira:2019, Newman:2018, Resende:2019}.

Acknowledging the distinct properties of many-to-many interactions, some recent studies have empirically analyzed them through the lens of {\it higher-order networks}, including 
%In the literature, these many-to-many networks have been commonly studied through models of \textit {higher-order networks} including
\textit{motif} (or graphlet) representations, \textit{multilayer} network, \textit{simplices} and \textit{hypergraphs} \cite{Meng:2018, Benson:2018, Liu:2019}. Those studies showed how the modeled phenomena exhibit rich and diverse patterns. For example, Benson et al.~\cite{Benson2:2018} explored  the structure of various of these networks, revealing a wide range of rich properties, such as, edge density and tie strength, which may vary according to the network context. They also investigated the higher-order link prediction problem, finding fundamental differences from traditionally studied pairwise link prediction. Higher-order link prediction  has also been studied by Meng et al.~\cite{Meng:2018}, who proposed a method to predict new interactions in groups (i.e., many-to-many interactions). The authors showed that the proposed method is significantly better than state-of-the-art models that consider predicting  pairwise links. In a different direction, other studies proposed strategies to model latent representations of higher-order networks. For example, Rossi et al.~\cite{Rossi:2018} proposed a general framework to learn higher-order network embedding representations  based on network motifs, evaluating it in the context of link prediction. With the same goal, others have used neural networks to extract latent patterns from signals to forecast the next sets of interactions from the previous ones \cite{Meng:2018, Hu:2019}.

Other recent studies have tackled the problem of detecting communities in higher-order networks by exploiting the presence of specific higher-order structures, that is, motifs. For example, Pizzuti et al.~\cite{Pizzuti:2017} employed a genetic algorithm to detect communities in networks formed by motifs, whereas Yin et al.~\cite{Yin:2017}, in turn, adopted a local graph clustering approach based on motif conductance. Tsourakakis et al.~\cite{Tsourakakis:2017} demonstrated the potential of methods based on motifs  for tackling clustering problems and graph mining, while Huang et al.~\cite{Huang:2019} proposed a motif-based community detection algorithm for higher-order multi-layer networks. Overall, these methods aim at uncovering communities that are based on particular structural patterns (i.e., motifs). 


In contrast, we are interested in revealing groups of users who are fundamentally responsible for the information dissemination process on Instagram. As such, these groups are not necessarily based on specific structural patterns (motifs) but rather are tightly connected subgraphs with respect to the rest of the network. Thus, the aforementioned techniques are not applicable, and we adopt a different approach. We  model the many-to-many interactions that occur among Instagram users as they comment on the 
same post by projecting them into a set of pairwise interactions. However, as argued by \cite{Benson:2018, Benson2:2018, Liebig:2016, Cao:2019}, such projected networks may include a large number of random and sporadic edges that are not really part of the fundamental underlying structure. Rather they occur mostly by chance or as a result of the superposition of multiple cliques of various sizes, representing the many-to-many interactions in the projected network.  Thus, we propose a generative model to filter such noisy edges out of the network before running further analyses.
%and then apply a widely used community detection algorithm to uncover communities in filtered network. Having uncovered these communities, we then analyze them with respect to different structural, content and temporal properties.

%\ju{The argument here is confusing. Need to revise whole paragraph after talking to Carlos.   why do we choose to work with the projection into pairwise interactions? Is this a result of the problems related to  the temporal analysis or is the cause of these problems? Not clear. What do you mean by temporally consistent but sporadic pattern?  I think it is missing the argument  of why these edges do NOT belong to the backbone. Finally, I still do not see why we could not use the algorithms for community detection in higher-order networks mentioned above? We need to clarify this. In sum, we must  justify the choice of model (as a set of pairwise interactions) and why aforementioned methods are not baselines.}
 
% \id{I agree with Jussara, this section is raising many questions. A reviewer will ask us to compare and validate our methodology against one of these alternatives after reading this. I would reduce this part to the very basic (less is more)... }

%Mudar para antes ... Mas parte já está na introdução.




%Regarding the detection of communities in these systems, we notice that vast majority of works considers static scenarios. Pizzuti et al.~\cite{Pizzuti:2017} employee a method for detecting communities in networks formed by motifs, through a genetic algorithm that minimizes metrics such as motif conductance. Similarly, Yin et al.~\cite{Yin:2017} adopt a local graph clustering approach based on motif conductance. In \cite{Tsourakakis:2017}, Tsourakakis et. al focus on methods based on motifs and demonstrate the potential of this structure for clustering problems and graph mining. In the work handled by Huang et al.~\cite{Huang:2019}, the authors extend the community detection based on motifs clustering to multilayer network modeling. In addition, ideas for latent vector representations based on embeddings have been studied since traditional methods exhibit difficulties in obtaining a representation of these structures in a vector space. Rossi et al.~\cite{Rossi:2018} aim to study connectivity patterns for link prediction. To the same end, others works use neural networks to extract latent patterns from signals to forecast the next sets of interactions through the previous ones \cite{Meng:2018, Hu:2019}. % Argumento do pq estamos utilizando o Louvain.


%Here, we capture the interactions among Instagram from the  many-to-many network structures to gain new insights into the community  organization from a co-commenting network built on Instagram by reducing them to a 2-projected graph \cite{XXX,YYY,ZZZ}. However, as explained by Benson et. al~\cite{Benson:2018}, when analyzed temporally, it is possible to notice prior co-interactions that appear repeated, new co-interactions are created from partial copies, partial co-interactions merges with earlier ones. These interactions cause the represented network to be composed of patterns that can be temporally consistent, but also sporadic, resulting in a rich but quite noisy topology. To address this, we project the sequence of many-to-many interactions and we propose a generative model to deal with network noise before detecting communities. After, we show how the emerging structure of the network reveals user behaviors previously not seen.
%Mudar para antes ... Mas parte já está na introdução.


\subsection{Network backbone extraction}
 %\ju[NAO e pra higher-order - os algoritmos nao foram definidos para projecoes de higher-order networks, embora tenham sido avaliados em redes de relacionamento binario e many-to-many (projecao).
 
 %Motivado por ruído, conexão esporádica, mas nao menciona many-to-many. 
 
 
 %CH: Por exemplo, suponha que 4 usuários sejam bastante ativos e alguns posts bastante popular em que esses 4 usários comentaram juntos. Grande parte dos modelos descritos a seguir consideraria que as arestas criadas entre eles salientes. Aqui no nosso modelo não. 
 %}
 
%As mentioned earlier, one key contribution of this article is a model to extract the network backbone from Instagram ecosystem based on many-to-many network, taking into account of its property such as media popularity and user activity level. Thus, the third body of work corresponds to those related to our proposal of employing a generative models suitable to extract the salient edges from a network formed through temporal many-to-many interactions. 

Network models and algorithms rely on the basic assumption that edges connecting nodes in the network faithfully represent the interactions that drive the phenomenon under study. Yet, there is an extensive debate on the consequences of ignoring data quality in such models since algorithms can be misled by the presence of noise in the network -- e.g., edges formed by random or sporadic interactions or even by measurement errors \cite{Slater:2009, Rahimi:2015, Newman:2018, Kobayashi:2019}. To address this problem, backbone extraction methods try to remove such noise and uncover a clearer image of the fundamental structure governing the network. These algorithms take as input the original network and provide a reduced version composed of {\it salient} edges, that is, edges that should more faithfully represent the phenomenon under study \cite{Coscia:2017}. 


Some of the simplest and most intuitive methods for removing edges explore topological metrics and properties of the graph. For example, some approaches rely on applying K-core searches for dense subgraphs and identifying hierarchical relationships among them~\cite{Sariyuce:2016, Savic:2019}. Another simple approach is based on setting a threshold for removing edges whose weights are smaller than a given value $\tau$. It has been widely used in several contexts, for example, biological networks \cite{Perkins:2009, Bordier:2017}, congressional voting networks \cite{Ferreira:2018}, financial networks \cite{Namaki:2011}, and online social networks \cite{Rahimi:2015}. This approach is particularly adequate when the salient edges are to some extent defined by the problem context (e.g., the edges with heavier weights in the network), making the use of a threshold principled \cite{Ferreira:2018, Yan:2018}. 


A somewhat different approach exploits the concept of neighborhood overlap, which reveals the tie strength between a pair of nodes in terms of the fraction of common neighbors. The intuition is that the network backbone should be composed only of ties (edges) with strength above a certain threshold. This approach has been applied, for example, to find polarized groups in congressional networks \cite{Ferreira:2019}, uncover research groups and collaborations in co-authorship networks \cite{Brandao:2017}, provide recommendations of places through the structure of the underlying network of contacts \cite{Valverde:2018}, and to address routing in a mobile ad-hoc network as a strategy to reach a reliable path among the various connections \cite{Gupta:2017}. However, some studies argue about potential misinterpretations of the results when using threshold-based approaches, as they could introduce biases in the analyses \cite{Tsur:2017}. For example, setting the threshold $\tau$ adequately is context-dependent and, as such, may be quite complex. Sometimes it is even not clear whether the same threshold $\tau$ should be applied to all edges \cite{Garrison:2015, Tsur:2017}.

  


%Another metric that is solely based on the topology of the graph is the neighborhood overlap, which reveals the tie strength between a pair of nodes in terms of their fraction of common neighbors. These techniques have been applied, for example, to find polarized groups in congressional networks \cite{Ferreira:2019}, to find research groups and collaborations in co-authorship networks \cite{Brandao:2017}, to study mobility, to provide recommendations of places through the structure of the underlying network of contacts \cite{Valverde:2018}, and to address routing in a mobile ad-hoc network as a strategy to reach out a reliable path by the various connections \cite{Gupta:2017}.


%A simpler alternative than to use to topological measures for extracting the network backbone is to set a threshold for removing edges whose weight is smaller than a given value \textit{w}. Indeed, it has been widely used in several contexts, for example, biological networks \cite{Perkins:2009, Bordier:2017}, congressional voting networks \cite{Ferreira:2018}, and online social networks \cite{Rahimi:2015}. However, some studies warn of possible misinterpretations and that these could result in a biased analysis \cite{Tsur:2017}. Choosing a threshold is a complex, context-dependent, sometimes being difficult to explain why an edge weighing less than \textit{w} should be removed. Nevertheless, in some problems the edge weight is explicitly expected and defined by the problem context, making the use of threshold approach principled \cite{Ferreira:2018, Yan:2018}. %However, such an approach could fail to capture the inherent heterogeneity of many complex systems where the formation of reducible links drastically varies in time and throughout the network

% more modern methods try to estimate the structure of the underlying network using statistical models, usually by defining a probability distribution \ju{of edge weights} in the  network and using it to define whether edges are removed or remain in the network based on the likelihood of their weights. Moreover instead of using a single probability distribution, many of these methods are based on local probability distributions, that is, specific to each edge or subset of edges of a given node \cite{Serrano:2009, Jacobs:2015}. 
% \ju{I think this description is wrong or misleading. the idea is that there is a reference model (a null hypothesis) and the probability distribution is defined under the assumption that the network is built according to this null hypothesis (uniform distribution across all edges of same node, poisson distribution, what?? Explain), and then, much like in a hypothesis test, you only keep edges whose weight pass the test.. Is that it? Need to explain this correctly.}

Recent approaches try to estimate the structure of the underlying network using statistical models. In particular, these methods assume a reference model describing how the network should be built under certain assumptions -- e.g., interactions occur by chance, based on independent behavior \cite{Jacobs:2015} or the weights of all edges incident to a node are uniformly distributed \cite{Slater:2009}. This reference model guides the definition of an edge weight distribution or even a generative process of the network, under the predefined assumptions. This distribution (or generative process) is used to filter out edges, leaving only those that deviate enough (in a probabilistic sense) from the given assumptions. For example, under the assumption of independent behavior, the authors of \cite{Silva:2014} filter out edges whose weights were below the $95^{th}$ percentile of the reference edge weight distribution. The intuition is that these edges may have been formed by pure chance under the assumption of independent behavior. In contrast, the remaining edges, whose weights are too large to be formed by independent behavior (i.e., with low probability - 5\%),  should represent interactions that are indeed relevant for the study and thus should be kept as part of the backbone. 

% Then, only edges whose weight pass the test remain in the networks \cite{Coscia:2017, Fornito:2016}. 

Rather than using a single probability distribution, some of these methods are based on local probability distributions, that is, specific to each edge or subset of edges of a given node. For instance, Serrano et al.~\cite{Serrano:2009} analyze whether a given edge bears a significant part of the total weight of a given node. Thus, edges are expressed as parts of the total edge weights of a node. These parts are then compared to a reference model, and $p$-values are used to determine how much an edge differs from it. The $p$-values are then used to prune the non-salient edges. Similarly, Coscia et al.~\cite{Coscia:2017} adopt a strategy that is based on whether or not an edge has a significant share of the total edge weight that enters from a given node, and then makes a statistical comparison with a reference model based on a random process. 



% The common goal of these methods is to extract the backbone from the network by removing what is regarded as non-salient edges. That is, edges arising from measurement errors, sporadic, random interactions and that somehow make it difficult to study a desired phenomenon.  \ju{Measurement error? Really? Are you sure?} \ch{Yes. In many networks the edges non-salient are from measurement errors.} Another marked property of these methods is to ensure that all the nodes have at least one connection \cite{Slater:2009, Newman:2018}. They assume that every node has at least one salient connection in the network on the hypotheses assumed. This means that the backbone extracted from the graph must have the same nodes as the original network. Conversely, other approaches do not guarantee that all original nodes will be present in the extracted backbone \cite{Serrano:2009, Grady:2012, Yan:2018}. Given these two perspectives, we argue that the might answer depends upon the problem and the method applied. For instance, it is important that the node remains connected to the network with at least one edge, as in the case of wireless sensor network such that all nodes need to be connected in the network \cite{Kumar:2020}. On the other hand, a node may not have any important edge that describes the phenomenon. For instance, highly polarized ideological groups formed by congressmen studied by a co-voting network at the House of Representative \cite{Ferreira:2018}, where the backbone not necessarily include all members. \ju{The second example is not clear. what does it mean for a congressman/node not to have any important edge? Who is this?? } \id{Make this part more direct. It is already going into the reasons for our method and departing from facts on the related work.} \ch{Done.}


Grady et al.~\cite{Grady:2012} proposed an alternative strategy that extracts the backbone network through a sampling process. This entails calculating the shortest path tree connecting the given node to all other nodes on the network. Then, the number of times that the edge appears in the paths is used to determine if it is or not salient. Note that if an edge was created at random but still plays an important structural role in the network, it is likely to be considered salient by this method. 

More recently, some authors have suggested extracting the network backbone taking into account temporal factors -- e.g., considering a sequence of snapshots of the network. For example, Kobayashi et al.~\cite{Kobayashi:2019} extract the backbone by exploiting a reference model based on the activity level of an edge in a sequence of snapshots.  Similarly, Nadini et al.~\cite{Nadini:2019} propose a model for detecting the backbone network by including temporal patterns of node interactions. 
Another family of methods focus on specific domains, trying to use contextual information to generate a domain-specific reference model. Examples include recommendation systems under online commercial networks~\cite{Zeng:2016}, urban mobility patterns~\cite{Manca:2017}, transportation networks~\cite{Wu:2006} and wireless sensor network~\cite{Kumar:2020}

As discussed previously, networks modeled from many-to-many interactions exhibit rich, diverse, but also noisy interactions. Unlike the aforementioned studies, we propose a novel generative model to extract backbones from co-commenters networks that reveals salient connections. It is based not only on principled statistical criteria built on the network structure, but also considering a different probability distribution for each edge in the projected network.  This distribution depends on the commenters' activity levels and on the number of opportunities they have to interact. In particular, our model provides an estimate for each edge to be considered salient, finally, revealing an underlying backbone.



==> 3_methodology_OLD.tex <==
\section{Methodology}
\label{sec:methodology}

In this section, we present the methodology used throughout our study. We start by formalizing the network of co-commenters on Instagram. Next, we introduce our probabilistic network model that is used to uncover salient interactions, that is, interactions that compose the network backbone. We then describe how we extract communities from the network backbone and present the techniques employed to characterize the temporal dynamics and the textual properties of the content associated with communities. % how we apply the Louvain algorithm to detect, characterize the temporal behavior of communities in the backbone networks, and analyze textual and psycholinguistic properties.

% \subsection{Terminology}
% \ch{The dataset section was moved to after the methodology. Maybe, we need to introduce the terminology of post, commenters, influencers according to that used in the two next subsections, \textit{network modeling} and \textit{Extracting the network backbone}.}

% \ch{I dont know if it is needed. The subsections here defined well the elements used. Set of Posts, weeks ...}


\subsection{Network of co-commenters}
\label{sec:netw}

%From each of the snapshots (i.e., 10 weeks of collected data), we build the networks that represent the interactions between commenters on posts of influencers.


%\textbf{XXX Explain why we define a week as the time interval XXX}.\mgm{done in sec.3}
We model the dynamics of interactions among commenters on Instagram posts as a sequence of snapshots, where each snapshot aggregates posts of a selected set of influencers as well as the comments associated with them over a fixed time window $w$. We here consider $w$ equal to one week, as we observe a large amount of interactions over such time period in our dataset. Moreover, we consider a week to be a reasonable period to cover discussions around posts, especially during election periods. % (as is the case in our dataset).

Given a time window $w$, we take the corresponding set of posts $P_w$, whose creation times fall within $w$, to create a weighted and undirected graph $G_w=(V_w,E_w)$. Vertices in set $V_w$ correspond to users who commented in  at least two posts in $P_w$. We choose to disregard commenters whose activities were concentrated on a single post and thus reflect very sporadic behavior.\footnote{Note that, by doing so, commenters who commented multiple times on a {\it single} post, but did not comment on other posts, are removed. For the purpose of identifying communities, we look at user commenting activity across different posts.}
%\ju{Carlos, is that correct? If the commenter posted N (N>>1) comments on a single post, you still remove it. Is that right?? Why?} \ch{Scalability} \fm{I would say that the algorithm could otherwise infer that the activities of such user are highly correlated with everyone else that commented on the same post.} \ch{We analyze the presence of these disregard commenters for each scenario and observe that between 91\% - 95\% of them comment at most three times within the analyzed period. In addition, we would like to prevent our model infers that the activities of such users are highly correlated with everyone else that commented on the same post.} 
Let $P_w(c) \subseteq P_w$ be the set of posts on which user $c$ commented. An edge $e_{cd} = (c,d)$ is added to set $E_w$ if $P_w(c) \cap P_w(d) \neq \emptyset$, i.e.,  commenters $c$ and $d$ commented at least once on the same post, which was shared during $w$. Thus, edges link co-commenters. The weight $\gamma({cd})$ of edge $e_{cd}$ is defined as the number of posts shared during window $w$ on which $c$ and $d$ commented together, i.e., $\gamma({cd}) =  |P_w(c) \cap P_w(d)| \in \{1,2,\ldots,|P_w|\}$.   % \ju{Carlos: what if $c$ and $d$ commented on a post that was posted during $w$ but their comments were posted AFTER w, meaning what defines the snapshots: the time of the post or the time of the comment???} \fm{I don't know, will have to wait for Carlos' answer}/ \ch{Here, we use the post creation time as criteria to define the snapshots. Thus, we consider all post comments regardless of whether they appear in the same week as the post or not.} 
%As we will present in Section \ref{sec:dataset}, our dataset covers posts of political influencers as well as other (general) influencers in two countries -- . Thus, 
Aiming at characterizing similarities and differences in discussions across different themes (political or not) and  countries (Brazil and Italy), we build a sequence of network models $\mathcal{G}=\{G_1, G_2 ... G_n\}$, where $n$ is the total number of time windows $w$, for each scenario.


%We model the dynamics of commenters in each temporal snapshot using graphs. Here, we consider snapshots aggregating posts and comments over one week because we observe a significant amount of interactions in this window size, but this could be flexible. Given a week $w$, we take the corresponding set of posts $P$ to create a weighted and undirected graph $G_P=(V_P,E_P)$. %\footnote{We drop the week index $w$ to simplify our notation.}
%We have a different $P$, and hence a different graph $G_P$, for each snapshot, country and category. The set of vertices $V_P$
%=$ $\{v_1, v_2,\ldots,v_n\}$
%represents commenters that commented in at least two posts in $P$.
%$E_P$
%=$ $\{e_1, e_2,\ldots,e_m\}$
%is the set of undirected edges, where there exists an edge $e_{cd}$=($c$, $d$) if commenters $c$ and $d$ commented in at least one common post in $P$. That is, edges link co-commenters. The weight $\gamma({cd})\in\mathbb{N}^+$ of edge $e_{cd}$ is defined as the number of posts where the co-commenters commented together, i.e., $\gamma({cd}) \in \{1,2,\ldots,|P|\}$.

Note that, as defined, each post $p$ in $P_w$ will generate a clique in the graph, i.e.,  a  subgraph where all pairs of vertices are adjacent. In other words,  each subgraph induced by a single post $p$ is complete by definition. The final network $G_w$  can thus be seen as the superposition of all the cliques generated by the posts in $P_w$. As such, $G_w$
results in a complex network, with several thousands of vertices and a large number of edges, many of which may be the result of  independent behavior of different commenters or may have occurred by chance (influenced by other factors rather than actual discussions). For example, a very popular post that attracted many commenters leads to 
a large clique in the graph. Yet, many co-interactions captured by  such clique are most probably  a  side effect of the popularity factor of the post (or the user who created it). Similarly, a user who is a very active commenter on a particular profile (commenting on many posts), will most probably co-occur as a commenter with many others. That is, such co-interactions are to some extent expected given their activity level.  Thus, to analyze interactions among co-commenters, we need to filter out such random and spurious edges, focusing rather on the edges that compose the fundamental underlying structure that defines the network of interactions under study, i.e., the \emph{network backbone}. %We present our approach to identify such edges in a given $G_w$ and extract its backbone in the next section.


%The network $G_P$ represents all interactions that happened among co-commenters on posts of a group of influencers during a week. $G_P$ results in a complex network with several thousand of nodes and even larges number of edges. In the following section, we show how to extract a more tractable and informative subgraph of $G_P$ that contains only its most important edges.

\subsection{Extracting the network backbone}
\label{sec:back}

Complex networks are non-random in many aspects. As such, a fundamental question that arises is how to quantify the statistical significance of an observed network structure with respect to a given reference graph model~\cite{Coscia:2017, Newman:2018}. Reference models are crucial in determining whether networks display certain features to a greater extent than expected by chance under a null hypothesis (e.g., independent behavior). A reference (or {\it null}) model matches some of the features of a graph and satisfies a collection of constraints, but is otherwise taken to be an unbiased random structure. It is used as a baseline to verify whether the object in question displays some non-trivial features, i.e., properties that would not be expected on the basis of chance alone or as a consequence of the constraints assumed. An appropriate reference model behaves in accordance with a reasonable null hypothesis for the behavior of the system under investigation. Rather than randomizing an existing network, reference models can be constructed by generative growing networks \cite{Easley:2010, Newman:2018}.

Our goal is to create a reference model $\widehat{G}_w$ from our network $G_w$, given the hypothesis that commenters behave independently from each other. We can then observe which edges of the real network do not behave in accordance with the reference model, that is, which edges reflect interactions that significantly deviate from an independent and random behavior. Such edges will compose the network {\it backbone}. The idea of the backbone is to capture only the \emph{salient} interactions, which are those that strongly suggest non-random interactions. Intuitively, we want to highlight those co-commenters who co-comment more frequently than what would be expected if they behaved independently.

We build a reference model $\widehat{G}_w$ in which edge weights are defined under a generative process in which commenters act independently from each other. However, their interactions with influencers' posts (i.e., which post each commenter comments on)  are not identically distributed. Our generative model takes into account the popularity of a post and the engagement of each commenter towards a given influencer. In other words, comments are randomly assigned to commenters preserving: i) the set of influencers on which each commenter writes a comment; ii) the popularity of the specific post (number of unique commenters) and iii) the engagement of each commenter towards an influencer, measured as the number of commented influencer's posts. By doing so, we prevent the backbone from being dominated by very active commenters or by those engaged in highly popular posts. Thus, our generative model takes as input the number of distinct commenters in each post ({\it post popularity}) and, for each commenter and influencer pair, the number of posts from each influencer the commenter commented on ({\it engagement}).  Using these statistics, the model assigns commenters to each post using independent and identically distributed (i.i.d.) draws from a distribution where the probability  is proportional to the commenter' engagement towards the influencer.  %\ju{Don't you need the total number of commenters as input?}


%\ju{ I think it would be good to give an abstract description of the generative model.  Given a post, what do we take as input? Number of commenters? Number of comments? Then we select a commenter based on which distribution -- WHy? Assumptions of the model. Tell the story, then move on to notation. Otherwise it is just too hard to understand, especially because notation is quite heavy} \fm{For parameter estimation, our generative model takes as input: the number of distinct commenters in each post (popularity) and the number of posts from an influencer that received comments from a given commenter (engagement), for each pair influencer-commenter. Based on these statistics, the model assigns commenters to each post using i.i.d.\ (independent and identically distributed) draws from a distribution where the probability of each commenter is proportional to her engagement towards the influencer.}

More specifically, let $I_w$ be the set of all influencers who wrote posts in $P_w$. Let $\mathcal{C}_p \subseteq V_w$ be the set of unique commenters in post $p \in P_w$ and $\{\mathcal{{P}}_w^i\}_{i \in I_w}$ be a partitioning of $P_w$ based on the influencer
$i \in I_w$ who created the post. We define the engagement of commenter $c \in V_w$ towards influencer $i$ (measured by the total number of posts in $\mathcal{P}_w^i$ commented by $c$) as
\begin{equation}
    x_i(c) = \sum_{p \in \mathcal{P}_w^i} \mathds{1}\{c \in \mathcal{C}_p\},
\end{equation}
%
where $\mathds{1}\{.\}$ is the identity function. We then  define $c$'s \textit{relative engagement} towards $i$ w.r.t.\ other commenters as:
\begin{equation}
f_i(c) = \frac{x_i(c)}{\sum_{d \in V_w} x_i(d)} = \frac{x_i(c)}{\sum_{p \in \mathcal{P}_w^i} |\mathcal{C}_p|}.
\end{equation}

%\ju{But $d$ was not defined in the summation. Give range! } \fm{I added the range and also an equivalent way to compute the denominator, used in the toy example.} 
In this way, we can describe in details the three steps of the generative model building our reference model~$\widehat{G}_w$:

\begin{enumerate}
    \item For each post $p \in P_w$, we consider a random assignment of each of the $|\mathcal{C}_p|$ (unique) commenters  to a commenter $c \in V_w$ with probability $f_i(c)$, where $i$ is the author of $p$. Specifically, under the assumption of independent behavior, we consider each such assignment as a Bernoulli random variable with parameter $f_i(c)$.  The probability that commenter $c$ is not assigned to $p$ is thus a Binomial random variable, with 0 successes in $|C_p|$ experiments. Conversely, under the assumption of independent behavior,  the probability that $c$ is a commenter (at least once) to a post $p \in \mathcal{P}_i$ is $r_p(c)=1-(1-f_i(c))^{|\mathcal{C}_p|}$.
    %    \ju{I think this sentence is wrong $C_p$ was defined as set of commenters, not comments.} \fm{This is the trickiest bit of the model. We counted multiple comments from the same commenter in a post as ``ONE interaction''. This is why we draw $|\mathcal{C}_p|$ times. However, we draw with replacement, because otherwise we would actually have to simulate in order to estimate the probability that each commenter is assigned to a post.} \fm{The number of comments to which $c$ is assigned follows a Binomial distribution}. \lv{Each comment is independent, hence we have $|C_p|$ draws of a Bernoulli random variable with parameter $f_i(c)$. The probability of commenter $c$ not being extracted  is expressed by a Binomial random variable, with 0 successes in $|C_p|$ experiments.} Hence, the probability that $c$ is assigned to at least one comment in $p \in \mathcal{P}_i$ is $r_p(c)=1-(1-f_i(c))^{|\mathcal{C}_p|}$.  \ju{Explain probability. Is this binomial?? Independent behavior. Link with assumption of null model.} %(We do not actually need to sample realizations of that assignment.)

    \item For each pair of commenters $c$ and $d$, we denote with $q_p(c,d)$ the probability that both get assigned to post $p$ and by $r_p(d|c)$ the probability that $d$ gets assigned to $p$ given that $c$ is assigned to $p$. The conditional probability $r_p(d|c)$ is necessary because, strictly speaking, although we are drawing commenters independently, when $c$ is drawn, it decreases the number of chances $d$ has for being drawn (since $|\mathcal{C}_p|$ is fixed). Hence, 
    $r_p(c,d) =   r_p(c) \times r_p(d|c).$
    %\begin{align*}
     %   r_p(c,d) = & \textrm{Prob(assigning $c$ as commenter of $p$) } \\
    %   & \times \textrm{Prob(assigning $d$ as commenter of $p$ | $c$ was assigned as commenter of $p$)}\\
    %    = & r_p(c) r_p(d|c).
    %\end{align*}
    %
    % \fm{To compute $q_p(c,d)$ exactly, we need to condition on the number of times one of the commenters is assigned to a comment in $p$ and then apply the total probability theorem:}
    % \begin{align*}
    %     q_p(c,d) & = \sum_{j=1}^{|\mathcal{C}_p|} \textrm{Pr(assigning $c$ to $j$ comments) $\times$ Pr(assigning $d$ to at least one of the $|\mathcal{C}_p|-j$ comments)}\\
    %     & = \sum_{j=1}^{|\mathcal{C}_p|} \binom{|\mathcal{C}_p|}{j} f_i(c)^j (1-f_i(c))^{|\mathcal{C}_p|-j} \times  (1-(1-f_j(c))^{|\mathcal{C}_p|-j})
    % \end{align*}
    %
    We approximate $r_p(c,d)\approx r_p(c)\times r_p(d)$, for each $p \in P$. Intuitively, this approximation works well when $|\mathcal{C}_p|$ is large (as in the case of most influencers' posts), because drawing $c$ decreases by only one the number of draws that can be used to draw $d$. Then, for each post $p\in P_w$, our model defines a distribution  over the set of vertices $\mathcal{C}_p$, where the value of the random variable $\widehat{\Gamma}_p{(c,d)} \in \{0,1\}$ indicating the existence of an edge between commenters $c$ and $d$ is given by a Bernoulli trial with parameter $r_p(c,d)$, i.e.\ $\widehat{\Gamma}_p{(c,d)} \sim \textrm{Bernoulli} (r_p(c,d))$. 

    \item The reference model $\widehat{G}_w=(\widehat{V}_w, \widehat{E}_w)$ is composed by the superposition of all the edges created for all $p \in P_w$. Hence, an edge $\widehat{e}_{cd} \in \widehat{E}_w$ will have a weight distribution described by a random variable $\widehat{\Gamma}{(c,d)} =  \sum_{p \in P_w} \widehat{\Gamma}_p{(c,d)}$. Therefore, it will be a sum of Bernoulli random variables with distinct probabilities \cite{Wang:1993}, which follows a Poisson Binomial distribution with parameters  $ r_1(c,d), r_2(c,d),\ldots,$ $ r_{|P_w|}(c,d) $.

\end{enumerate}


With the reference model $\widehat{G}_w$, we can then compare it with the observed network ${G}_w$ to extract the backbone $B_w$ of the latter. We do so by keeping in $B_w$ only
%Comparing the two graphs, we create the backbone graph ${B}_P$ of the original ${G}_P$ networks by considering only
edges of ${G}_w$ whose weights have values exceeding the ones expected in $\widehat{G}_w$ by a large margin. Specifically, for each edge $\widehat{e}_{cd}$ we compute the $(1-\alpha)^{th}$ percentile, denoted by $\widehat{\gamma}_{1-\alpha}(c,d)$, of the distribution of edge weight $\widehat{\Gamma}(c,d)$, and compare it with the observed edge weight ${\gamma}{(c,d)}$. We keep edge $e_{cd}$ in the network backbone if ${\gamma}{(c,d)} > \widehat{\gamma}_{1-\alpha}{(c,d)}$. Intuitively, we keep only edges between co-commenters who interacted much more often than expected under the assumption of independent behavior, that is, edges for which the  chance of such frequency of interactions  being observed under the independence assumption is below $\alpha$. We here choose to set $\alpha$ = 5\%, as done in several prior studies \cite{Serrano:2009, Kobayashi:2019}. Note that, after filtering out edges as described, isolated vertices are also removed.  At the end, we extract from the network $G_w$ its backbone $B_w= (V^b_w, E^b_w)$ where $V^b_w \subseteq V_w$ and
$E^b_w \subseteq E_w$.

% \mt{why 1-alpha? could we set directly alpha to 0.95?}
%under the independence assumption, would be observed in fewer than 5\% of cases.

Note that the $(1-\alpha)^\textrm{th}$ percentile is computed separately for each edge $e_{cd} \in E_w$ from  random variable $\widehat{\Gamma}(c,d)$. For such a Poisson binomial distribution, there is a closed form for computing a given percentile and it relies on a combinatorial computation~\cite{Hong:2013}. Since this is expensive to compute exactly, we use the Refined Normal Approximation (RNA)~\cite{Hong:2013}, a method that proved very good performance with low computational complexity.

To illustrate how our model works, we consider a toy example with three commenters ($c$, $d$ and $e$) who interact with each other by commenting on posts of 2 influencers ($i$ and $j$). In total, we consider $|P_w| = 7$ posts. Figure \ref{Fig:toy_example}a shows a co-interaction matrix where rows represent commenters ($c$, $d$ and $e$) and columns represent posts. The number of distinct commenters who commented on each post $p$, given by $\mathcal{C}_p$, is shown on the bottom of the figure.  Figure \ref{Fig:toy_example}b shows the network of co-commenters built from these data.

%use the following toy example. Figure \ref{Fig:toy_fig_1} shows a co-interaction matrix such that two Influencers ($i$ and $j$ $\in$ $\mathcal{I}$) have together $|p| = 7$ posts. We highlight three commenters $c$, $d$ and $e$ $\in$ $\mathcal{U}_p$, that commented on some of the seven posts. The member of distinct commenters that comment at least once in post $p$ is given by $\mathcal{C}_p$. For the sake of simplicity, we focus on the commenters $c$, $d$ and $e$, but notice that the total of commenters $C_p$ for each post $p$ can be larger than shown in the matrix except.


% \begin{figure}[h]
%     \centering
%     \subfloat[Co-interaction Matrix]{\includegraphics[width=0.25\columnwidth]{fig/toy_fig_1.png}\label{Fig:toy_fig_1}}\hspace{0.5cm}
%     \subfloat[Corresponding  Network]{\includegraphics[width=0.18\columnwidth]{fig/toy_fig_2.png}\label{Fig:toy_fig_2}\vspace{0.2cm}}
%     \caption{Toy example from the Instagram interaction: Commenters on  7 posts by 2 influencers.} \label{Fig:toy_example} %\lv{in Fig.1a, why the three points? It is an example with 7 comments and 3 commenters. Remove the three points. Also $C_p$ is wrong...are there more than 3 commenters? } \ch{No Luca. This Figure is a part of interactions and there are more commenters than 3 (c,d,e). So, the three points are necessary and $C_p$ is greater than 3 for some posts. Otherwise, the toy example doesnt work. Final version, tiny details like this one can be solved. But, for me it is ok.}
% \end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.55\columnwidth]{fig/Fig1.pdf}\label{Fig:toy_fig_3}
    \caption{Toy example from the Instagram interaction: Commenters on  7 posts by 2 influencers.}\label{Fig:toy_example}
\end{figure}

Following the three steps defined above, we first compute the relative engagement $f$ of each commenter towards each influencer.  The relative engagement is the probability that a commenter gets assigned to a given comment of the influencer under the reference model, and is given by:
%
\begin{equation*}
\small
\begin{aligned}[c]
f_i{(c)} = \frac{3}{3+2+3+3} = \frac{3}{11} = 0.27,
\end{aligned}
\qquad
\begin{aligned}[c]
f_i{(d)} = \frac{2}{11} = 0.18,
\end{aligned}
\end{equation*}

\begin{equation*}
\small
\begin{aligned}[c]
f_i{(e)} = \frac{1}{11} = 0.09,
\end{aligned}
\qquad
\begin{aligned}[c]
f_j{(c)} = f_j{(d)} = f_j{(e)} = \frac{1}{7} = 0.14.
\end{aligned}
\end{equation*}
For clarity, let's define $\widehat{C}_p$ the set of commenters randomly assigned to post $p$. The probability that a commenter belongs to $\widehat{C}_p$ depends on the number of distinct commenters in the data, $|C_p|$. Given the relative engagements $f$, computed as described above, these probabilities are given by:
%
\begin{center}
$r_1(c) = \textrm{Prob}(c \in p_1) =  (1 - (1-0.27)^3) = 0.61$   

$r_1(d) = \textrm{Prob}(d \in p_1) =  (1 - (1-0.18)^3) = 0.44$

$\vdots$

$r_7(e) = \textrm{Prob}(e \in p_7) =   (1 - (1-0.14)^3) = 0.36$
\end{center}

The last step is to approximate the theoretical distribution of weights according to a Poisson Binomial distribution with parameter vector $\mathbf{r}(c,d) = (r_1(c,d), \ldots, r_{|P_w|}(c,d))$ for each pair of commenters $(c,d)$, defined as: 

\begin{center}
$r_1(c,d) = \textrm{Prob}(c,d \in p_1) = 0.61 \times 0.44 = 0.26$ 

$\vdots$

$r_7(c,d) = \textrm{Prob}(c,d \in p_7) = 0.36 \times 0.36 = 0.12$
\end{center}
%
Thus, the theoretical distribution of weight for each edge $(c,d)$ is
%
\begin{equation}
\nonumber
\widehat{\Gamma}^{(c,d)}= \widehat{\Gamma}^{(c,d)}_{p_1} + \widehat{\Gamma}^{(c,d)}_{p_2} + ... + \widehat{\Gamma}^{(c,d)}_{p_7}, \textnormal{such that } \widehat{\Gamma}^{(c,d)}_{p} \sim  \textrm{Bernoulli}(r_p(c,d)).
\end{equation}
%
That is, $\widehat{\Gamma}^{(c,d)}$ has Poisson Binomial distribution with parameter vector $\mathbf{r}(c,d) = \left(r_1(c,d), \ldots, r_{7}(c,d)\right)$. 
We use this distribution to filter out edges for which the independent behavior assumption cannot be rejected. Precisely, we keep those edges whose weights are above the corresponding threshold of significance -- chosen as the $95^\textrm{th}$ percentile ($1-\alpha$ = 95) of the edge weight distribution under the independence assumption ($\widehat{\gamma}_{95}{(c,d)}$). We illustrate this process in Figure \ref{Fig:toy_example_2}, which shows three graphs: the original network $G_w$, a graph with edges labeled with corresponding thresholds, and the resulting backbone $B_w$. In this example,  edge $e_{cd}$ is not salient  and is thus removed from the backbone.  Moreover, after filtering out  $e_{cd}$, the vertex $d$ becomes isolated and is thus removed. The final backbone consists of only edge $e_{ce}$. 
% \ju{This figure is hard to follow. I suggest to label each edge in each graph with whatever you are showing, using the notation defined above, you do have notations for the observed edge weight as well as for 95th percentile of the null model. This will make it easier to understand.} \fm{Great suggestion! Will have to wait for Carlos, though.}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.75\columnwidth]{fig/Fig2.png}\caption{Comparison of the original (observed) graph with the reference model for the extraction of the backbone.}\label{Fig:toy_example_2}
\end{figure}

% In this section, we describe the model proposed and exemplified how it works by a toy example. Then, the next steps of the methodology aim to understand how the communities of commenters are formed on the backbone and their temporal and textual proprieties.


\subsection{Detecting communities in a network backbone}
\label{sec:communities}

%Now that we have a clearer image of the network (the backbone ${B}_P$) with only the edges we are interested to study, we want to group together the nodes according to their relationships.

Once extracted the backbone $B_w$ from the network $G_w$, we want to identify communities in $B_w$. Qualitatively, a community is defined as a subset of vertices such that connections between such vertices are denser than connections to the rest of the network. To extract communities from $B_w$, we adopt the widely used Louvain algorithm~\cite{Blondel_2008,Newman:2004}.
 % widely used for community detection in networks~\cite{Pujol, greene}. Communities are non-overlapping sets of nodes in the graph.
The goal of the Louvain algorithm is to maximize the modularity of the communities, where modularity quantifies the quality of assignments of vertices to communities. Intuitively, the modularity captures how much densely connected the vertices within a community are, compared to how connected they would be in a random network with the same degree sequence. Modularity is defined in the range of -1 to +1, and modularity scores of 0.5 or higher are considered strong evidence of well-shaped communities.
%Specifically, modularity is a measure between -1 and +1 that captures how much higher/lower is the density of edges inside communities in comparison to a network with the same degree sequence but where nodes are randomly connected. Modularity of 0.5 or higher is considered a  solid indication of well-shaped communities.
Since trying out all possible communities is computationally impractical, several heuristic algorithms have been proposed. The Louvain method is one of these, and it operates by finding first small communities optimizing modularity locally on all vertices. Then, each small community is merged into one meta-vertex and the first step is repeated.
%Modularity measure the quality of division of a network into  communities. Its values range from -1 to 1 such that a high modularity have dense connections between the nodes within communities and sparse connections between nodes in different communities.
The final number of communities is the result of an optimization procedure. In other words, given the graph $B_w = (V^{b}_w, E^{b}_w)$,  the Louvain algorithm extracts the set of communities that provides the highest modularity value. For a weighted graph, the modularity is defined as:

$$ Q={\frac {1}{2M}}\sum \limits _{c,d \in V^b_w}{\bigg [}\gamma({cd})-{\frac {k({c})k({d})}{2M}}{\bigg ]}\delta (\ell({c}),\ell({d}))$$

where
\begin{itemize}
\item $\gamma(c,d)$ is edge weight between vertices $c$ and $d$ ($e_{cd} \in E^b_w$);
\item $k(c)$ and $k(d)$ are the sum of the weights of the edges attached to vertices $c$ and $d$, respectively, in $B_w$;
\item $M$ is the sum of all of the edge weights in $B_w$ ;
\item $\ell({c})$ and $\ell({d})$ are the communities assigned to $c$ and $d$; and
\item $\delta$ is the Kronecker delta function, i.e.,   $\delta({\ell({c}),\ell({d})})=1$ if $\ell({c})=\ell({d})$,  $0$ otherwise.
\end{itemize}

We refer the reader to~\cite{Blondel_2008} for a detailed description of the Louvain algorithm.

\subsection{Characterizing communities}
\label{sec:textual}

We characterize the communities extracted from the network backbones in terms of i) the content associated with each community, i.e., textual properties of the comments posted by its members, and ii) the temporal dynamics of community membership.

\subsubsection{Content properties}


%\subsection{Analyzing textual and psycholinguistic properties}

%The popularity of social media has changed the way people communicate with each other and share knowledge, how companies advertise their products, and how politicians  debate and influence their constituents. Consequently, the availability of  numerous methods and methodologies for analyzing the properties of online content, mainly textual content, has enabled deeper investigations of how people interact with each through the analysis of their digital footprints\cite{Sapountzi:2018}. In this article, we aim at characterizing the communities extracted from the network bacbkones in terms of content, how commenters interact among them and how the psycholinguistics properties differentiate them from each other.


% To accomplish it, we start by \textit{\textbf{T}erm \textbf{F}requency–\textbf{I}nverse \textbf{D}ocument \textbf{F}requency} (TF-IDF) analysis for revealing words able to describe community in relation to the others \cite{Jones:1972}. Given a document collection $D$, TF-IDF starts measuring the significance of words in a document $d \in D$. To do it, the first step is to compute $TF(t,d)$ for each document $d$ meaning how frequent is a term $t$ present in this document in all document collection:
% \begin{equation}
%     TF(t,d) = \left(\frac{\textnormal{\# times term $t$ appears in the document $d$}}{\textnormal{\# total of terms in the document $d$}}\right)
% \end{equation}
%  %
% and $IDF(t,d,D)$ indicates the importance or degree of distinction of term $t$ within the whole document collection:
% %
% \begin{equation}
%     IDF(t,d,D) = \log_2\left(\frac{\textnormal{\# total of documents}}{\textnormal{\# documents with term $t$}}\right)
% \end{equation}

% Here, a document is formed by all comments carried out by a given community. The comments are pre-processing such that all their terms are transformed to lowercase, stop words, emojis, punctuation, and single characters are removed. Last, the lemmatization process is used to reduce the term to root synonym (e.g. plural words to singular). The documents are represented in a vector space where each document $t$ present in a document $d$ of document collection $D$ receive the weight:
% %
% \begin{equation}
%     TF-IDF_{(t, d, D)}=\mathrm{tf} (t,d)\cdot \mathrm{idf} (t,D)
% \end{equation}

% From this representation we can extract the most discriminate words ranking the TF-IDF score for each document. In additional,  it is possible to check the similarity between two document representation to check, for instance, how similar two communities are in terms of content computing the Cosine Similarity metric among the vector space $u_{(d_1}$ and $v_{(d_2)}$ representing two given documents $d_1$ and $d_2$, as follow:
% %
% \begin{equation}
% \cos(u_{(d_1)}, v_{(d_2)}) = 1 - \frac{\mathbf{u}_{(d_1)} \cdot \mathbf{v}_{(d_2)}}{
% \|\mathbf{u}_{(d_1)}\| \|\mathbf{\mathbf{v}}_{(d_2)}\|}.
% \label{eq:cos}
% \end{equation}
% %
% Cosine distance ranges from 0 to 1, where values close to 0 indicate that the documents are very distinct in terms of words while values close to 1 indicate that the documents are completely similar.

%\subsubsection{TF-IDF to understand topic}

We characterize the textual properties of the comments of members of each community using three complementary approaches. First, we use sentiment analysis on comments of each community. Second, we run a TF-IDF analysis~\cite{Jones:1972} to reveal terms that characterize each community. Finally, we use the \emph{Linguistic Inquiry and Word Count} (LIWC) tool~\cite{Tausczik:2010} to delve deeper into the psycholinguistic properties of the terms used by members of each community. Overall these approaches allow us to offer a picture on similarities and differences across communities, helping us in finding the peculiarities of their discourses.

For the sentiment analysis, we apply SentiStrength,\footnote{\url{http://sentistrength.wlv.ac.uk/index.html}} a lexical dictionary labeled by humans with multi-language support, including Portuguese and Italian. Given a sentence defined as a comment, SentiStrength classifies its sentiment with a score ranging from -4 (extremely negative) to +4 (extremely positive). Scores equal to 0 indicate neutral sentiment~\cite{Thelwall:2010}. SentiStrength has been widely applied to analyze the sentiment of textual content posted on social networks and, notably, of short texts with a very particular language including abbreviations (e.g., tweets) for which identifying sentiment is usually harder~\cite{Ribeiro:2016, Thelwall:2017}. 

The \emph{Term Frequency - Inverse Document Frequency} (TF-IDF) technique \cite{Jones:1972} allows us to select terms that characterize each community. TF-IDF is traditionally used to describe \emph{documents} in a collection with the most representative terms. Given a particular term and a document, the TF-IDF is computed as the product of the frequency of the term in the given document ($TF$) and the inverse of the frequency at which the term appears in distinct documents ($IDF$). Whereas $TF$ estimates how well the given term describes the document (i.e, terms that appear more often in a document tend to better describe its content), $IDF$ captures the term's capacity to discriminate the document from others. Good document representations are composed by terms that meet a trade-off between these two quantities.
%computed for each word  on a collection of \emph{documents} by calculating a metric that takes into account the frequency each word appears on each document ($TF$) and the inverse of the frequency the word appears on distinct documents ($IDF$).
To apply TF-IDF in our context, we represent each community as a {\it document} consisting of all comments of the community members. We pre-process the comments using \emph{spaCy}\footnote{\url{https://spacy.io/}} to i) keep only verbs, adverbs, nouns and proper nouns; ii) remove emojis, stopwords, hashtags, punctuation and mentions to other users; iii) perform lemmatization; iv) transform text to lowercase; and v) remove the overall top-1\% most popular terms, and those words that appear less than 10 times. The former are words whose frequency is extremely high (e.g., word \textit{election}) and would not help to characterize the communities. The latter are mostly typing errors or grammar mistakes.

Each community is then represented by a vector $d$ with dimension equal to the number of unique terms in the collection. The element $d[i]$ is the TF-IDF of term $i$. In our particular case, however, the classic definition for $IDF$ is not appropriate as we have a small number of documents, unlike in its traditional use for information retrieval \cite{Baeza:1999}. Most terms appear in the majority of documents, leading to small and mostly similar values of $IDF$. For that reason, we use an alternative definition  called probabilistic inverse document frequency, defined as $IDF(i)=\log \frac{N-n_i}{n_i}$, where $N$ is the total number of communities and $n_i$ is the number of communities using the term $i$ \cite{Baeza:1999}. This variation is more sensitive to small changes on $n_i$, thus increasing discrimination in our case. We manually evaluate the terms with large TF-IDF on each community searching for particular subjects of discussion and discourse. Moreover, we assess the similarity between the content produced by different communities by computing the cosine similarity of the corresponding vectors \cite{Baeza:1999}. That is, the similarity between communities $j$ and $k$ is defined as  $sim_{jk} = d_j \times d_k$. Note that  $sim_{jk}$ ranges from $0$ (maximum dissimilarity) to $1$ (maximum similarity). 


% where $1$ means the vectors have the same components and $0$ means there is no term $i$ such $d_j[i] \neq 0 \land d_k[i] \neq 0$, i.e., $d_j$ and $d_k$ are orthogonal.

% Being TF-IDF non negative by construction, cosine distance ranges from 0 to 1, where values close to 0 indicate that the documents are very distinct in terms of words while values close to 1 indicate that the documents are completely similar. However, one TF-IDF \id{??} Since the term frequencies (using TF–IDF weights) cannot be negative. However, depending on the normalization to be applied in the IDF, it can be negative, allowing it to cosine similarity ranges from -1 to 1.  \ju{This paragraph is very confusing. Need to be rewritten. There is a sentence that seems to be missing a part. Not sure why do you say that cosine can be -1?? What noramlization was applied?  Need to specify here and why it leads to -1. If it does not, do not mention it, and just give the right range.}

%\subsubsection{SentiStrength to gauge sentiment}


%It is known for doing so in a very conservative way in relation to entries that do not have a clear sentiment, classifying them as neutral .
% \ju{ I did not understand the last sentence. What is the point being made here??? Is this good or bad? Does it tend to output neutral more often (than what?) Not sure.}

%\subsubsection{LIWC for psycholinguistic analysis}

Last, we delve deeper into the properties community comments using LIWC~\cite{Tausczik:2010}, a lexicon system that categorizes text into psycholinguistic properties. Words of the target language are organized as a hierarchy of categories and subcategories that form the set of LIWC attributes. Examples of attributes include linguistic properties (e.g., articles, nouns and verbs), affect words (e.g., anxiety, anger and sadness) and cognitive attributes (e.g., insight, certainty and discrepancies). The hierarchy is customized for each language, with 64 and 83 attributes for Portuguese and Italian, respectively.

When presenting results, we translate all attributes to English, even if they are encoded in the original language in LIWC. We apply LIWC to each comment of each community to quantify the fraction of words in the comment that falls into each attribute. By analyzing these fractions, we can identify attributes that characterize comments of a community. However, not all attributes appear in a comment. In addition, given an attribute, we are interested in knowing whether its frequency is significantly different for comments made by the various communities. We search for statistical differences across communities based on the average frequencies of their respective attributes. We first use Kruskal's non-parametric test to select only attributes for which there is a significant difference across communities~\cite{Kruskal:1952}. Then, we rank attributes with significant differences to select the most discriminative ones using the Gini Coefficient \cite{Yitzhaki:1979}. 

% to selected the top-5 attributes with the highest coefficient, that are those with the greatest variation between communities.



%a psycholinguistic text analysis tool. LIWC calculates the degree to which various categories of words (e.g., \ju{XX, XX,XX}) are used in an input document.

%Here, we used the versions of the LIWC for Portuguese and Italian. LIWC takes as input a document and returns the percentage of words in each pre-defined attribute categories. These categories help us to understand, for instance, style, effective and cognitive behavior behind the document. In total, there are 92 LIWC attributes. The percentage value of a given attribute is normalized to the input size, in our case, a comment.

%\ch{Examples will be used in the results section. So, we can pick up example to the attributes selected. Also, I dont know if we need to explain here the methodology part where we did a test of hypotheses, etc. What do you thing? Does the statistical part should be here or in the result section?}

\subsubsection{Temporal Dynamics}
\label{sec:metho_tempo}

We also want to analyze how communities evolve, in terms of their memberships, over consecutive time windows. To this end, we compute two complementary metrics. The first metric,  \textit{persistence},  captures the extent to which commenters that are part of the backbone at window $w$   remain in (some community of) the backbone at window $w+1$.  In other words, the persistence at time window $w+1$ is measured as the fraction of commenters in $B_w$ who are present in $B_{w+1}$. If persistence is equal to 1, all commenters in $w$ are still present in $w+1$ (plus eventually others). Yet, the membership of individual communities may have changed as members may have switched communities.


%belonging to some community of backbone $B_w$ remain in (some community in) backbone $B_{w+1}$. . Given the week $w$, the persistence in  $w+1$ measures the fraction of commenters in the backbone of $w$ who are present in the backbone of $w+1$. If persistence is equal to 1, all commenters in $w$ are still present in $w+1$ (plus eventually others). Yet - their membership to individual communities can change.

To capture changes in community membership, we compute the \emph{Normalized Mutual Information} (NMI) over the communities~\cite{Lancichinetti}, taking only commenters who persisted over  consecutive time windows.  NMI is based on Shannon entropy of information theory \cite{Shannon:2001}.
Given two sets of partitions $X$ and $Y$ defining community assignments for vertices in weeks $w$ and $w+1$, the mutual information of $X$ and $Y$ represents the informational overlap between $X$ and $Y$, or, in other words, how much we can learn about $Y$ from $X$ (and about $X$ from $Y$). Let $P(x)$ be the probability that a vertex picked at random is assigned to community $x$, and $P(x,y)$ the probability that a vertex picked at random is assigned to both $x$ in $X$ and $y$ in $Y$. Let $H(X)$ be the Shannon entropy for $X$ defined as $H(X)=-\sum_x P(x) \log P(x)$. As such, the NMI of $X$ and $Y$ is defined as:
%
\begin{equation}
NMI(X,Y)=\frac{\sum_x \sum_y P(x,y)\log \frac{P(x,y)}{P(x)P(y)}}{\sqrt{H(X)H(Y)}}
\end{equation}

NMI ranges from 0 to 1 where 0 implies that  all commenters changed their communities and  1 implies that all commenters remained in the same community.  We compute NMI at each time window $w+1$  by taking the sets of communities identified in windows $w$ and $w+1$, considering, as mentioned, only members who persisted from the backbone $B_w$ to the backbone $B_{w+1}$. 


==> 6_results_textual_OLD.tex <==
\section{Community behavior}
\label{sec:rq2}

In the previous section, we observed that some communities share interest on the same influencers, differing on the subset of posts they comment more heavily. We now address the second research question, focusing on how the communities differ from each other in terms of textual, sentiment and psychological properties of comments. To this end, we use the methodologies and techniques described in Section~\ref{sec:textual}. 

% First, we investigate the behavior of these community the sentiment of the comments. After, we extract discriminative words from communities comments to gain insights into what communities commenting. Last, we delve into the meaning of these words reflect using a lexicon dictionary.

\subsection{Political communities' interests}

%As observed in the previous section, communities comment on different influencers. Here, we delve deeper into how communities are attracted by posts.
We begin by looking into how communities in politics are attracted by different posts. Since communities differ in the number of members and in the number of comments they post, we consider a relative \emph{interest index} of a community for a post, given by the fraction of the community's comments that belong to the post. We illustrate the way the community interest is distributed across posts using data from the week of the main elections in Brazil (week 5). Figure~\ref{fig:Activity}a quantifies, for each post, the two most interested communities in the post. The $x$-axis reports the index for the community with highest interest for the post, while the $y$-axis reports the index for the second most interested community in the post. 

% Similar comments hold true for the Italian case.
%\fm{Can we state something short about Italy's?}

We observe that in some cases the most interested community made 7\% of its comments in a unique post (see the $x$-axis). Given there are $2\,144$ posts in this snapshot, even a relative interest of 1\% can be considered a highly concentrated attention, suggesting that communities are built around specific posts. In almost 40\% of the posts, the relative interest of the second most interested community ($y$-axis) is very low compared to the most interested community. This last observation is illustrated in Figure~\ref{fig:Activity}b, which reports the ratio between the relative interests of the first and the second most interested communities (note x-axis log-scale). We observe that often the most interested community has at least 10 times higher index than the second one.

\begin{figure*}[!t]
        \includegraphics[width=0.7\columnwidth]{fig/Fig7.png}
        \caption{Interest of communities on posts.}
        \label{fig:Activity}
\end{figure*}

Figure~\ref{fig:examples} shows examples of posts that attracted high interest for communities $3$ and $7$, which we use as running examples along with communities $10$ and $11$. We observe that community $3$ comments mostly on posts related to public events Bolsonaro promoted via Instagram (Figures~\ref{fig:examples}a and Figures~\ref{fig:examples}b), while community $7$ comments on posts where the candidate tries to show his proximity with black people to debunk his associations with racism (Figures~\ref{fig:examples}c and Figures~\ref{fig:examples}d).


\begin{figure*}[!t]
\includegraphics[width=0.98\columnwidth]{fig/Fig8.png}
\caption{Examples of posts by Jair Bolsonaro (jairmessiasbolsonaro) in which two communities show high interest.}
\label{fig:examples}
\end{figure*}

\subsection{Properties of communities' comments}

% \ch{\textbf{What has been done?}
% \begin{itemize}
%     \item In the section of dataset characterization (section 3) we show a lot of metrics about the dataset. So, a question that aroused was: How does link this section with the communities results? Here we extend this characterization to community level in order to observe particular behavior on communities found. 
%     \item To summarize the characterization for all communities of all weeks, we compute the same metrics used in the section 3 for each community found and compute one unique PCA for all weeks and all scenarios, that is, BR-Politcs, IT-Politics, BR-General and IT-Politics.
%     \item The 3 figures with PCA below show, respectively: a) the communities position in the latent space for all Scenario and all weeks. In an overview, there is no strong difference between communities belonging the same scenario, but there is a more significant difference among scenarios. After, b) and c) show that is no clear difference among communities found in the election week and other snapshots. I dont know if Figure b) and c) should be continue. Notice that for the three figures, the same PCA was used. That is, only one PCA was computed.
%     \item Also, there is a figure showing what features compose the two components and a table to describe the feature's name. 
%     \item Last, in the separate figure (the one that appear after the figure of applicability of the features), there is another possible PCA analysis that could be performed. But again, I don't know if there are any interesting finding. 
    
% \end{itemize}}

We now take each community found in each snapshot and extract properties of the comments of their members, namely: 1) Average comment length (in characters); 2) Fraction of comments that include at least one mention; 3) Average number of hashtags per comment; 4) Fraction of comments with at least one uppercase word; 5) Average number of comments per commenter; 6) Average number of emojis per comment; and 7) Fraction of replies among comments. 
% To obtain a comprehensive view of the communities behavior unveiled by our methodology, we take each community found in all snapshots and all scenarios, look at the comments carried out by the commenters belonging these communities, and compute: 1) Average characters by comment; 2) Fraction comments that have at least one mention; 3) Average number of hashtags in a comment; 4) Fraction comments with at least one uppercase word; 5) Average number comments per commenter; 6) Average number emojis in a comment; 7) Fraction of replies among comments.
Together these metrics may capture important aspects of the communities' behavior. For example, the comment length, the number of emojis per comment and the use of uppercase words (commonly associated with a high tone) can describe the way the communities interact on Instagram. Mentions, the use of hashtags and replies are strongly associated with engagement, information spreading and direct interaction of commenters, respectively.

We obtain a 2-D representation of the communities by applying Principal Component Analysis (PCA) to vectors that represent communities using the seven previously described metrics. PCA is a well-known method for dimensionality reduction in multivariate analysis. It projects the data along its principal components (PCs), i.e., axes that capture most of the variance in the data~\cite{Tipping:1999}. Figure~\ref{Fig:PCA}a shows the representation obtained for each community using the two principal components, where the color represents the pair country-scenario. The 2-D representations of communities for both politics scenarios are more tightly clustered and overlapping than for the general scenario. This behavior suggests that, when considering the given features, communities on politics are more homogeneous than the communities on the general scenario.

% , regardless of country, are mostly tightly overlapped representing a cohesive behavior. Yet, communities belonging the general scenario exhibit a larger variation as showed by the 2D representation and are slightly overlapped with politics scenario. In essence, according to the metrics we can observe difference of behavior, between politics and general influencers.   



To understand which metrics best distinguish the communities in Figure~\ref{Fig:PCA}a, we study the \emph{loading scores} for the two principal components. The loading score quantifies the contribution of each metric to a principal component. The largest the score (in absolute value) the more the metric contributes to the component (positively or negatively).

%Positive values indicate that a higher (resp.\ lower) than average value of that metric contributes positively (resp.\ negatively) to the component's coordinate. On the other hand, a negative loading score indicates that a higher (resp.\ lower) than average value of that metric contributes negatively (resp.\ positively) to the component's coordinate. Therefore, the largest loading scores (in absolute value) show the metrics that most contribute (positively or negatively) to each component.

% It means that the more negative loading score in the bar, the lower the metric's absolute values and, therefore, the more to the left the point is located in the 2-D representation in Figure \ref{Fig:PCA}. If the ``loaded score'' is positive, the opposite is observed. Also, the more extreme bar values, whether negative or positive, the more discriminatory is the metric observed. For instance, the most extreme value in the component 1 is the average number of characters in a comment and it is positive. In this way, the more right points (communities) in the Figure \ref{Fig:PCA} indicates that these communities carried out comments with a higher average number of characters. Notice that the communities more to right correspond to the politics scenarios. 

\begin{figure}[!h]
\includegraphics[width=0.98\columnwidth]{fig/Fig9.png}\label{Fig:PCA}
\caption{(a) 2-D representation of communities based on seven metrics using PCA. (b) Description of the two principal components in terms of the original metrics; The bar represents the loading scores for the components (positive or negative).}
    
    % \caption{...\mgm{This shall go before the community defintion part. It's still the characterization of the dataset. Here we need to redo the same plots, but dots are now communities, and not snapshots. Use the same PCA for projections. Are communities different in terms of the way people comment? Color of community can refer to the top influencer (i.e., political party as done in fig 8)}\ch{These PCAs are in relation to communities. Figura a), each point is a community, independent of snapshot (All communities for all snapshots are represented)). It shows that the communities of a given scenario have some variation in terms of how they comment, but the greatest variation occurs between the scenarios. Figures b) and c) show that the communities of the elections week have no differences in relation to the communities of the other weeks for Brazil and Italy, respectively. Let go to the next Figure try to do something different.}\mgm{Ok - I missed that each point is a community, for each snapshot. Better to be clear here :)}}
\end{figure}

In Figure~\ref{Fig:PCA}b bars represent the magnitude of loading scores for each metric for the PC 1 (left) and PC 2 (right). The PC 1 (left) can be associated with lengthy comments, high usage of uppercase, emojis, replies and hashtags, and a low number of comments per commenter. From Figure~\ref{Fig:PCA}a, we see that high values for PC 1 is more common for communities in the politics scenarios. Conversely, most communities of the general scenario have negative $x$ coordinates, thus pointing to a different behavior.

% Focusing at the component 1, it is possible to observe that it is explained mainly by the average number of characters in a comment and the fraction comments with uppercase words. Therefore, the communities more right in Figure \ref{Fig:PCA}, which are politics one, do longer comments and use more uppercase words. Similarly, the other metrics show that politics communities use more hashtags, emojis and reply more. Conversely, most communities of the general scenario are located to the left having opposite behavior.

A less clear picture emerges for PC 2. Large values for the PC 2 are associated with high numbers of replies, mentions and comments per commenter (see Figure~\ref{Fig:PCA}b, right plot). For the politics scenario in Figure \ref{Fig:PCA}a, communities are concentrated in the $y \in [-2,3]$ range, with those for Italy being slightly more positive than those from Brazil. In the general scenario, however, points are spread out along the $y$ axis. 

% The distribution of the values along PC 2 does not change much between countries, although the points for a few communities from Italy take on higher positive values.

% is associated we can see that it is explained mostly by the fraction of comments with mentions, the fraction of replies among comments, and by the average number of comments by commenter. Accordingly, the communities upper at the y-axis in Figure \ref{Fig:PCA} mention more, reply more and their commenters comment more. In general, there is no large difference between communities from general and politics scenario in both countries. However, we can see again a more variability in communities of general scenario while the politics one in more concentrated. Remember that the general scenario is composed of diversified kinds of influencers and, then, it is expected a larger behavior variation within it. 

In short, we conclude that commenters of politics influencers exhibit a more homogeneous behavior than commenters of communities related to other influencers.

\subsection{Sentiment analysis}
\label{sec:sentiment}


% \ch{Methodology for Sentiment Analysis: We compute the sentiment using sentistrength in all comments and analyzing from different view.
% \begin{enumerate}
%     \item We start analyzing the fraction of each sentiment in each scenario here studied. There are a table with the respective fraction and a graph with the distribution for each scenario and the distribution. In the last meeting, we decided to use only the distributions. So the table are useful to put the number in the caption or in the text. The justification for using SentiStrenght is that it is multilanguage and have been applied on OSN's. 
    
%     \item Remember that we have a lot of graphs contrasting communities with an influencer, communities with communities ... and so on. Once that we decide to remove neutral of analysis, the simplest and most efficient visualization found was the heatmap. First, in order to avoid that community with very few comments in a given profile generates biased visualization, we ignored communities with less than 100 comments in a given profile. Then, we plotted two heatmaps, one for positive and other for negative sentiment considering the respective sentiment for each community on each top influencers. It is possible to see interesting visualizations comparing with the heatmaps Figure 6, such as communities with a higher fraction of negative sentiment in the opposite candidates. We need to be very careful in to claim that more negative comments in a profile indicates crude speech about the candidate because a comment can support a candidate by saying negative things in his post, but speaking negatively about another candidate. 
    
%     \item Another analysis made was in relation to the conditional sentiment of comments that have any reply. To do it, we compute for a given comment its sentiment and the sentiments of all comments that are replies of this respective comment. They are 4 graphs, one for each scenario, showing the fraction of sentiment for a reply according to the sentiment of the original comment. In short, in politics, there are more negative comments (Table below), and theses negative sentiments exalt negative responses.
% \end{enumerate}}

Although communities grow around particular posts and influencers, we saw that their members do comment on posts from many other influencers. Here, we analyze whether there is a difference between the sentiment expressed in comments according to the influencers. As explained in Section~\ref{sec:methodology}, we use SentiStrength to extract the sentiment of each comment. SentiStrength provides a score ranging from -4 (strongly negative) to +4 (strongly positive). Score 0 implies a neutral sentiment. We here consider as \emph{negative}, \emph{neutral} and  \emph{positive} comments with scores smaller than 0, equal to 0, and greater than 0, respectively. 

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.72\columnwidth]{fig/Fig10.png}
    \caption{Distribution of sentiment captured on comments for each scenario. We use red for negative, gray for neutral and green for positive comments.}
    \label{fig:distribution-sentiment}
\end{figure}

Figure \ref{fig:distribution-sentiment} shows the distribution of the sentiment score for each scenario, while Table~\ref{tab:fraction-comments} concisely reports the fraction of positive, neutral and negative comments. We notice that positive comments are generally more common (between 47\% and 58\%), followed by neutral comments (between 32\% and 41\%). We look into the neutral comments to understand why they represent a significant fraction and observe a large number of short comments, misspelled words, abbreviations etc, which seem to complicate sentiment extraction by SentiStrength. Negative comments are the minority in our data, but they are more prevalent in the politics scenarios for both countries.


\begin{table}[!h]
\caption{Fraction of sentiment captured in comments using SentiStrenght.}
\begin{tabular}{cccc}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Scenario}}} & \multicolumn{3}{c|}{\textbf{Sentiment}}                                                                                 \\ \cline{2-4} 
\multicolumn{1}{|c|}{}                                   & \multicolumn{1}{c|}{\textbf{Negative}} & \multicolumn{1}{c|}{\textbf{Neutral}} & \multicolumn{1}{c|}{\textbf{Positive}} \\ \hline
\multicolumn{1}{|c|}{BR Politics}                        & \multicolumn{1}{c|}{0.10}              & \multicolumn{1}{c|}{0.32}             & \multicolumn{1}{c|}{0.58}              \\ \hline
\multicolumn{1}{|c|}{IT Politics}                        & \multicolumn{1}{c|}{0.13}              & \multicolumn{1}{c|}{0.40}             & \multicolumn{1}{c|}{0.47}              \\ \hline                                                                                                                                                          \hline
\multicolumn{1}{|c|}{BR General}                         & \multicolumn{1}{c|}{0.06}              & \multicolumn{1}{c|}{0.41}             & \multicolumn{1}{c|}{0.53}              \\ \hline
\multicolumn{1}{|c|}{IT General}                         & \multicolumn{1}{c|}{0.04}              & \multicolumn{1}{c|}{0.36}             & \multicolumn{1}{c|}{0.57}              \\ \hline
\end{tabular}
\label{tab:fraction-comments}
\end{table}

Next, we analyze how the communities' sentiment varies towards profiles of different politicians. More specifically, we compute the breakdown of positive, neutral and negative comments of each community on posts of each influencer. Similarly to the complete scenarios (see Table~\ref{tab:fraction-comments}), the breakdown stratified by community and influencer shows more positive than negative comments. To summarize differences, we report in Figure~\ref{Fig:sentiment_BR} and Figure~\ref{fig:sentiment_IT} a \emph{contrastive score} calculated as the difference between the fractions of positive and negative comments for the particular community and influencer. We ignore cases where a community has made less than 100 comments on a given influencer's posts to ensure that samples are representative. These cases are marked as white cells in the heatmaps shown in the figures.

We consider in Figure~\ref{Fig:sentiment_BR} 6 influencers on the week of the first election round in Brazil (week 5). Predominantly, communities make positive comments on the profiles in which they are more active, i.e., their ``referring candidate''. More negative comments are seen on ``opposing candidates''. For instance, communities 1 to 9, highly active on Jair Bolsonaro's posts, display a more positive contrastive score on them. Analogously, communities 10 to 12, mostly formed by commenters very active on the profiles of left-wing influencers such as Ciro Gomes (cirogomes) and Fernando Haddad (fernandohaddadoficial), tend to write negative comments on their opponents, such as Jair Bolsonaro. This behavior is seen across the heatmap and suggests that communities in politics tend to promote their central influencers, while trying to demote others.

\begin{figure}[t!]
\centering
\includegraphics[width=0.60\columnwidth]{fig/Fig11.pdf}
\caption{Contrastive sentiment score (difference between fraction of positive and negative comments) of communities towards political leaders during the main election week in Brazil (week 5).}
\label{Fig:sentiment_BR}
\end{figure}

% The Figures \ref{Fig:Dist_Sentiment_Comm_BR} show the distribution of positive and negative sentiment for each community in the first election round for Brazil. We disregard communities that commented less than one hundred times on an Influencer to avoid bias in the viewing. Each cell in the heatmap corresponds to the fraction of the comments with the respective sentiment considering only the comments performed by the community on the respective Influencer. That is, the sum of the corresponding cells in the positive (Figure \ref{Fig:Postive_BR}), negative (Figure \ref{Fig:Negative_BR}) and neutral (ignored) is equal to one.
% \textbf{\ch{Stop here...}}

% Essentially, we note that communities make more positive comments under the profiles that they are more active and more negative comments under the profiles that they are less active. For instance, focusing in communities from 1 to 9, strongly active on Jair Bolsonaro (jairmessiasbolsonaro) profile, we can notice in Figure \ref{Fig:Postive_BR} that they comment more positively on his profile and more on the others. Yet, Figure \ref{Fig:Negative_BR} shows that these same communities comment less negatively on his profile. In a more specific example, observe Community 1, mainly, in terms of negative comments. It is possible to see that it comments more in a negative way on the other influencers' profiles than in the Bolsonaro one. Similarly, looking at the communities from 10 to 13, more attacked for left-wing influencers such Ciro Gomes (cirogomes), Fernando Haddad (fernandohaddadoficial) and Lula (lulaoficial) the same pattern is observed. This behavior extends across all heatmap and indicates that communities in politics tend to comment more positively on influencers that they interact predominantly and more negatively on the others. %This behavior became more noticeable in all the heatmap when contrasted with Figure \ref{Fig:hetmaps_br} where we can see under which Influences each communities are more and less active.


% \begin{figure}[!t]
%     \centering
%     % \subfloat[Positive]{\includegraphics[width=0.50\columnwidth]{fig/journal/BR-politics-HeatMap-Positive-V1.pdf}\label{Fig:Postive_BR}}
%     % \subfloat[Negative]{\includegraphics[width=0.50\columnwidth]{fig/journal/BR-politics-HeatMap-Negative-V1.pdf}\label{Fig:Negative_BR}}\\
%     \subfloat[Brazil]{\includegraphics[width=0.50\columnwidth]{fig/journal/sentiment_merged_BR.pdf}\label{Fig:dsadsa}}
%     \caption{Fraction of positive sentiment minus the negative sentiment among political leaders and communities during the main election weeks in Brazil.}
%     \label{Fig:Dist_Sentiment_Comm_BR} %\textbf{Brazil\mgm{may be we can use the same colors for incluencers according to their political coalition - as done in fig 8.} \ch{It is easy and fast to do, but I don't know if it will bring viewing gain. In the Brazilian case, only fernandohaddad and lulaofficial are from the same party (One replaces the other during the running.). In relation to Italy, is there some pattern that brightens? Also, as color is related to sentiment, it will be generate a color overlapping. For instance, in Brazilian fernandohaddad and lulaofficial should be red and alvarodias green, respecting their political parties and ideologies. }\mgm{I was just referring to put names in the x-axis with colors - as done in fig.8. Cells would be the same. :) }
% \end{figure}

Considering the Italian case, we observe similar results in Figure~\ref{fig:sentiment_IT}: communities exhibit positive contrastive scores towards candidates in general, but with higher scores for the referring candidate.




% \begin{figure}[!h]
%     \centering
%     % \subfloat[Positive]{\includegraphics[width=0.50\columnwidth]{fig/journal/IT-politics-HeatMap-Positive-V1.pdf}\label{Fig:Positive_BR}}
%     % \subfloat[Negative]{\includegraphics[width=0.50\columnwidth]{fig/journal/IT-politics-HeatMap-Negative-V1.pdf}\label{Fig:Negative_BR}}\\
%     \subfloat[]{\includegraphics[width=0.50\columnwidth]{fig/journal/sentiment_merged_IT.pdf}\label{Fig:dsadsa}}\\
%     % \subfloat[Positive]{\includegraphics[width=0.50\columnwidth]{fig/journal/IT-politics-HeatMap-Positive-V2.pdf}\label{Fig:Comm2_BR}} 
%     % \subfloat[Negative]{\includegraphics[width=0.50\columnwidth]{fig/journal/IT-politics-HeatMap-Negative-V2.pdf}\label{Fig:Comm2_BR}}
%     \label{Fig:Dist_Sentiment_Comm_IT}
%     \caption{Fraction of comment sentiment on a subset of influencer in the electoral week for Italy.}
% \end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.60\columnwidth]{fig/Fig12.pdf}
\caption{Contrastive sentiment score (difference between fraction of positive and negative comments) of communities towards political leaders during the main week of the European election.}
\label{fig:sentiment_IT}
\end{figure}

%Up to now, we notice that the sentiment behind of the comments exhibits the great variation among influencers and also that the fraction of comments with replies is an important characteristic present in the communities, mainly in politics.
Finally, we check also the relationship between the sentiment of a comment and the replies it receives. Remind that commenters can reply directly to comments previously left on a post. Figure~\ref{Fig:Replies_Sentiment} shows, for all scenarios, the frequency of the reply sentiment ($S_r$), given the original comment sentiment ($S_c$). Neutral comments and replies are not depicted. When comments are positive, they tend to attract at least twice as many positive replies as the negative ones. While negative comments still attract mostly positive replies, their numbers decrease significantly, especially for the politics scenario. In other words, negative comments attract higher numbers of negative replies than the positive comments. 

% \id{This section ends in a big "so what". This figure can go away.}

% More negative comments are observed, mainly in the political context for both countries. This indicates that the debate in the political context is even more severe when stimulated. %We also looked for negative comments on influencers that are not politics, that is, the general scenario, and notice that many negative comments are observed for influencers from sport context and in cases of solidarity and health campaigns whose sentences are guided by negative words.



\begin{figure}[h]
\centering
\includegraphics[width=0.58\columnwidth]{fig/Fig13.png}
\caption{Fraction of replies of each sentiment conditioned on comment sentiment. }\label{Fig:Replies_Sentiment} 
\end{figure}


\subsection{Textual properties}
\label{sec:res_textual}

% \ch{Methodology of TF-IDF Analysis:
% \begin{enumerate}
%     \item For each scenario an analyze was did such that: For each community, we created a document grouping all comments carried out by the commenters of the respective community building the corpus. For instance, in the Brazil week election we have 13 communities, there are 13 documents composing our corpus. 
    
%     \item In a pre-processing, emojis, stop words, mentions links and hashtags were removed, and lowercasing was applied. Then, we characterized the word frequency of the corpus e remove words that appears less than 10 times. They are in the vast majority types and grammar mistakes. Filtering out these not frequent words, we remove approximately 70 percent of the words for our four corpus. Also, we use only verbs, adverbs, noun and proper noun. To do this filter, we used e Spacy natural language processing toolkit multilanguage that works for Portuguese and Italian languages. The methodology details should be put in the methodology section.
    
%     \item From the pre-processing, we ran TF-IDF and compute: 1) The document similarity using cosine distance, plotted in the heatmaps. 2) The top 10 words more representative according to the TF-IDF metric for each document(community) in the political scenarios. For the general, we picked up 5 communities and selected the top 10 words more representative.
% \end{enumerate}}

We now turn our attention to the textual properties of comments. As before, we focus on the election weeks. To summarize the overall behavior of each community, we group together all their respective comments in one document. As explained in Section \ref{sec:methodology}, the documents build a corpus on which we then use the TF-IDF metric to identify the most representative words of each document (i.e., community), henceforth called \emph{top words}.

First, we analyze the top words for political communities. Due to the large number of communities, we discuss only those yielding the most interesting observations. Table~\ref{tab:political-words} shows the top-10 words (translated to English) for a selection of communities. We manually inspect the comments and related posts, providing a reference context as the last column of the table. The manual inspection suggests that these words give a good overview of what the communities discuss. 

Matching with what is seen earlier in Figure~\ref{fig:examples}, communities 3 and 7 for Brazil are associated with rallies in different locations in the country, and with debunking Bolsonaro's prejudice against ethnic and racial groups. The terms highlighted by TF-IDF reflect quite accurately the respective topics, reporting locations of rallies and words linked to racism and Nazism. Similarly, the top words for communities 10 and 11 are focused on the names of the candidates whose profiles they mostly comment on. For Italy, community 3 reflects the typical jargon used by Salvini's supporters. Community 4 debates on taxes and monetary issues. Community 10's comments refer to provoking posts that mix taxes, car costs and animals' rights. Last, community 11 seems to debate over left-wing party (the main opposition party at the time) and the 5-Stars movement (the governing party at the time). 








\begin{table}[h]
\tiny
\caption{Example of words with the highest TF-IDF for some communities in the politics scenario in the main election week.}
\label{tab:political-words}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Scenario} & \textbf{Comm.} & \textbf{Key Words}                                                                                                                              & \textbf{Context}                                                                                                                                                           \\ \hline
BR  & 3                  & \begin{tabular}[c]{@{}c@{}}`Anapolis', `Orla', `Righteousness', `Constant', \\ `Natal',  `Paulista', `Spontaneous', \\ `JB17', `Gesture', `Avenue' \end{tabular} & \begin{tabular}[c]{@{}c@{}}It refers to several places \\where pro-Bolsonaro rallies  took \\ place during the election campaign.\end{tabular}                                    \\ \hline
BR  & 7                  & \begin{tabular}[c]{@{}c@{}}`Nazi', `Jew', `Hitler', \\ `Black People', `Anonymity', `Bozonazi', \\`Distrust', `Jerusalem', `Homosexual' \end{tabular}          & \begin{tabular}[c]{@{}c@{}}It refers to Bolsonaro's posts about \\ specific social groups in an attempt to show \\ he has no prejudice against such groups.\end{tabular} \\ \hline

BR  & 10                  & \begin{tabular}[c]{@{}c@{}}`Manuela', `Haddad, `Scammer', \\ `Lulalivre', `Birthday', `Guilherme', \\ `Dilma', `Gratefulness', `Lula'\end{tabular}          & \begin{tabular}[c]{@{}c@{}}It refers to left-wing names, \\ such as Fernando Haddad,  his \\ deputy Manuela, Dilma Rousseff and Lula (ex-presidents).\end{tabular} \\ \hline

BR  & 11                 &
\begin{tabular}[c]{@{}c@{}}`Ciro', `Experience', `Political Activism', \\ `Polarization',  `Brazil', `Second Round', \\`Turn', `Prepared', `Project' \end{tabular}    & \begin{tabular}[c]{@{}c@{}}It refers to the center-left candidate \\ Ciro Gomes  who arrived close to \\reach the second round of the elections.\end{tabular}                                                                                          \\ \hline
IT  & 3                  & \begin{tabular}[c]{@{}c@{}}`Gooders', `Big ciao'', `Captain', \\`Crime', `Good night', `Polls', \\ `Never Give Up', `Electorate', `Lampedusa', `Riace' \end{tabular} & \begin{tabular}[c]{@{}c@{}}General Salvini's jargon, \\as well as places  related to \\the arrival of immigrants in Europe (e.g., Lampedusa).  \end{tabular}                                                                                                        \\ \hline
IT  & 4                  & \begin{tabular}[c]{@{}c@{}} `Monetary', `Elite', `Unity', `Budget',\\ `Fiscal', `Colonial', `Equalize', \\`Yellow Vests', `Masonic', `Store', `IVA', \end{tabular} & \begin{tabular}[c]{@{}c@{}}Generic taxes and monetary issues.\end{tabular}                                                                                                        \\ \hline
IT  & 10                  & \begin{tabular}[c]{@{}c@{}}`Consumption', `Fuel', `Insurance', `Traffic',\\ `Helpless', `Vehicular', `Taxes', `Redundancy', \\`Veterinary', `Animal rights', `Cats', `Abuse', `Cruelty', `Breeding'\end{tabular} & \begin{tabular}[c]{@{}c@{}} A combination of terms related\\ to taxes, vehicles and animals' rights.\end{tabular}                                                                                                        \\ \hline
IT  & 11                  & \begin{tabular}[c]{@{}c@{}}`5S', `Toninelli (ex-Transport Minister)', `Corruption',\\ `Zingaretti (PD's leader)', `Calenda (ex-PD politician)', \\`Honesty', `Election list', `Coalition', `Budget', `Growth'  \end{tabular} & \begin{tabular}[c]{@{}c@{}}Debate on Five Stars Movement (a government\\ party at the time) and Democratic \\Party (the main opposition party at the time)\end{tabular}                                    \\ \hline
\end{tabular}
\end{table}




%\fm{I am assuming you use a vector with the same dimension as the vocabulary and then zero the entries that are not in the top-100, so that all vectors are comparable, right?}. \ch{Yes}.
 
Next, we compute the cosine similarity between the TF-IDF representations of documents. Given the large size of the vocabulary, we consider only the top-100 words with the highest TF-IDF scores in each document, zero-ing other entries in the TF-IDF vectors. Figure~\ref{Fig:Heatmaps} shows the similarity matrix as a heatmap for each of the four scenarios. In the heatmap, we sort communities to place similar ones next to each other. By doing so, groups of similar communities are evident along the main diagonal. In general, for all scenarios, we find that communities use rather distinct vocabularies -- i.e., the cosine similarity is very low -- as testified by the predominance of the blue shades indicating similarity values below 0.2. This is not surprising given that TF-IDF was designed to pinpoint the most \emph{discriminative} terms. However, we find a few blocks with high similarity, unveiling the communities whose top words have more intersection. 

In particular, for the politics, Figures \ref{Fig:Heatmaps}a and \ref{Fig:Heatmaps}b highlight one group of 3 similar communities, for both Brazil and  Italy. Manually inspecting the top 25 words for communities 5, 8 and 9 in Brazil, we observe indeed some common words -- e.g., \textit{Good Morning,\footnote{Originally a single word before translation} Coffee, Kitchen, Pan and Sink}. Looking at the posts where they appear, we found some posts from Bolsonaro featuring pictures in which he appears making coffee in his kitchen\footnote{See e.g., \url{https://www.instagram.com/p/BojIGjUHsQO/}}. The three communities turn out to be very active on these same posts, albeit formed by distinct commenters. We observe the same behavior on the Italy - politics scenario, where a single block with communities 12, 13 and 14 appears on the top-left corner of the figure. We also check the intersection between their top terms, which, however, turn out to be very generic words -- e.g., \textit{to go, to be, stay strong, to stay and to see}. These are small communities that make very few comments. Most words from the vocabulary never appear in these communities' comments, yielding very sparse TF-IDF vectors. However, the presence of generic terms combined with small normalization constants (i.e., product of the TF-IDF vectors' norms) result in high cosine similarity values. Yet, these terms do not reveal interesting properties shared by the communities.

Moving on to the general scenario, Figures~\ref{Fig:Heatmaps}c and \ref{Fig:Heatmaps}d show some groups of communities sharing a similar lexicon. Manual inspection reveals that these are small communities for which TF-IDF has difficulty to pinpoint interesting terms -- the majority of them being generic terms (or expressions, when translated) such as \textit{Good Morning}, \textit{Good Night}, \textit{Amazing}, \textit{Loving}, \textit{Beautiful}. 


\begin{figure}[!t]
    \centering
    \includegraphics[width=0.78\columnwidth]{fig/Fig14.png}
    \caption{Cosine Similarity among community comments. For both countries, snapshots during main election weeks were considered.}\label{Fig:Heatmaps}
\end{figure}


%\mt{Maybe we could remove tf idf for the general case. The text says these results are not good...}\ana{agree} \ch{Now, it is late to do it. Several changes and something can become broken.}

In a nutshell, the TF-IDF is instrumental to analyze what the communities are discussing -- when there are naturally emerging topics. When communities are too generic or too small, TF-IDF provides little insights. The analysis demonstrates that some communities are quite representative of the political debate, even if they have been built solely based on commenters' interactions without accounting for the content of comments.



% \begin{table}[h]
% \scriptsize
% \caption{BR - Politics - Top 10 words\mgm{why don'twe use a cloud word representation - and pick just some examples of communities? Then we can put all cloudtags to a techrep - or in an online page. cloudtags can also show the weitght (tfidf score) of the word.
% another possible visualization: Create a graph with words as nodes, links if they appear in the same community. node size can be tfidf. Color of nodes identifies a community. Link weight can be the product of tfidf scores of two nodes - or similar.  Put this in gephy, and let it place nodes. this would allow to show both words, communities, and common words - if any.}\ch{Nice ideas. I think that the wordcloud idea is still better, because we already showing the similarity and differences between communities' vocabulary in the heatmap before. I need to experiment with how wordcloud works for so few words for each community.}\mgm{ok - may be generate separate worldclouds - one for each community - may fit the case. One worldcloud with multiple communities may be more complicated tought. }}


% \begin{tabular}{|c|c|}
% \hline
% \textbf{Community} & \textbf{Key Words}                                                                                                                                        \\ \hline
% 1                  & \begin{tabular}[c]{@{}c@{}}Round, Joice, Bolsonaro, Carla,\\ Manipulation, Photography, Flavio,\\ Brazilian, Press, Inhibit\end{tabular}                  \\ \hline
% 2                  & \begin{tabular}[c]{@{}c@{}}Round, Debate, Surgery, Sofa, \\ Colostomy, Belly, Living room, Stab, Lesion\end{tabular}                                      \\ \hline
% 3                  & \begin{tabular}[c]{@{}c@{}}Maceió, Crawl, Bolsonaro, Motorcade, Paulista Avenue, \\ Exciting, Brazilian, Espirito Santo, Panic, Brazil\end{tabular}       \\ \hline
% 4                  & \begin{tabular}[c]{@{}c@{}}Capitan, Round, Recovery, Rest, \\ Bolsonaro, Strength, Bless, Beautiful, Day\end{tabular}                                     \\ \hline
% 5                  & \begin{tabular}[c]{@{}c@{}}Coffee, Table, Sink, Rest, Recommendation, \\ Simplicity, Relaxing, Surgery, Strainer, Theater\end{tabular}                    \\ \hline
% 6                  & \begin{tabular}[c]{@{}c@{}}Distract, Slapped, Make up, Intolerant, Sexual, \\ Beat, Makeup artist, Beautiful, Crawl, Quality\end{tabular}                  \\ \hline
% 7                  & \begin{tabular}[c]{@{}c@{}}Racist, Jewish, Nazism, Homosexual, Problems,\\ Administrative, Suspect, Highlight, Anonymity\end{tabular}                     \\ \hline
% 8                  & \begin{tabular}[c]{@{}c@{}}Sink, Bolsonaro, Coffee, Round, To wash, \\ Shirt, Support, Smell, Mistake\end{tabular}                                        \\ \hline
% 9                  & \begin{tabular}[c]{@{}c@{}}Coffee, Captain, Crockery, Good Morning,\\ Sink, Kitchen, Strength, Evening, Myth\end{tabular}                                    \\ \hline
% 10                 & \begin{tabular}[c]{@{}c@{}}Manuela, Boulos, Birthday, Haddad, Companion, Squid, \\ Fascist, Hitting, Missing, Injustice\end{tabular}                      \\ \hline
% 11                 & \begin{tabular}[c]{@{}c@{}}Ciro, Experience, Political Activism, Polarization,\\ Brazil, Second, Round, Turn, Prepared, Project\end{tabular}              \\ \hline
% 12                 & \begin{tabular}[c]{@{}c@{}}Zema, People, Pimentel, Anastasia, Marina, Debate,\\  Deforestation, Life trajectory, Sustainability, Environment\end{tabular} \\ \hline
% 13                 & \begin{tabular}[c]{@{}c@{}}Sergipe, Police Chief, Renovation, Senate,\\ Surveillance, Coherence, Criticize, Clean Slate\end{tabular}                      \\ \hline
% \end{tabular}
% \end{table}




% \begin{table}[h]
% \scriptsize
% \caption{BR - General - Example of 5 communities. Put the Italy General here.}
% \begin{tabular}{|c|c|}
% \hline
% \textbf{Community} & \textbf{Key Words}                                                                                                                          \\ \hline
% 10                 & \begin{tabular}[c]{@{}c@{}}Gay, Singer, Woman, Preconception, Pablo,\\ To respect, Alok, Globo TV Channel, Trash, Malhação TV Show\end{tabular}     \\ \hline
% 22                 & \begin{tabular}[c]{@{}c@{}}Shirt, Gift, Brazil, Shame, Corinthians, Cheat,\\ Soccer match, To respect, Northeast, Arbitration,\end{tabular} \\ \hline
% 25                 & \begin{tabular}[c]{@{}c@{}}Medicine, Register, Surgery, Donor, Need,\\ To help, Kid, Collaboration, Urgency\end{tabular}                    \\ \hline
% 28                 & \begin{tabular}[c]{@{}c@{}}Amen, Provide, To pray, Rosary, Love, To bless, \\ Job, Unemployed, Family, Faith\end{tabular}                   \\ \hline
% 30                 & \begin{tabular}[c]{@{}c@{}}Coffee, Friend, Laugh, Good, To Give\\ Love, Beautiful, Life, Affection, Stay\end{tabular}                       \\ \hline
% \end{tabular}
% \end{table}






% \begin{table}[h]
% \scriptsize
% \caption{IT - Politics - Top 10 words}
% \begin{tabular}{|c|c|}
% \hline
% \textbf{Community} & \textbf{Key Words}                                                                                                                                        \\ \hline
% 1                  & \begin{tabular}[c]{@{}c@{}}Salvini, Country, Poor, Home,\\ Christian, Left-Wing, Church, Bishop, Dead, Live\end{tabular}                  \\ \hline
% 2                  & \begin{tabular}[c]{@{}c@{}}Salvini, Guilt, Country, Left-Wind,\\ Liberal, Home, Grace, Poor, Unemployment, Dock\end{tabular}                                      \\ \hline
% 3                  & \begin{tabular}[c]{@{}c@{}}Salvini, Crime, Minister, Country, Grace,\\ Friend, Change, Block, Answer\end{tabular}       \\ \hline
% 4                  & \begin{tabular}[c]{@{}c@{}}Elite, Nigeria, Home, Expel, Money,\\ Fiscal, Colony, Oligarchy, Confiscate\end{tabular}                                     \\ \hline
% 5                  & \begin{tabular}[c]{@{}c@{}}Salvini, Mediate, Social Class, Christian,\\ Transport, Corruption, Immigrant, Enter, Office, Determination \end{tabular}                    \\ \hline
% 6                  & \begin{tabular}[c]{@{}c@{}}Salvini, Christian, Guilt, Church, Priest,\\ Bishop, Nutella, Grace, Pedophilia, Dock\end{tabular}                  \\ \hline
% 7                  & \begin{tabular}[c]{@{}c@{}}Salvini, Church, Christian, Computer,\\ Fuchsia, Change, School, Mininster, Dock, Country\end{tabular}                     \\ \hline
% 8                  & \begin{tabular}[c]{@{}c@{}}Salvini, Country, Dock, Arrive, Poor,\\ Faith, Reason, Grace, Justice, Home\end{tabular}                                        \\ \hline
% 9                  & \begin{tabular}[c]{@{}c@{}}Salvini, Network, Donation, Grace, Minister,\\ Christian, Poor, Territory\end{tabular}                                    \\ \hline
% 10                 & \begin{tabular}[c]{@{}c@{}}Animal, Dog, Mistreat, Insurance,\\ Fuel, Liter, Circulation, Janitor, Government\end{tabular}                      \\ \hline
% 11                 & \begin{tabular}[c]{@{}c@{}}Desert, Corruption, Immunity, Honest,\\ Minister, Undersecretary, Euro, Contract\end{tabular}              \\ \hline
% 12                 & \begin{tabular}[c]{@{}c@{}} Antifascism, Communism, Left-Wing,\\ Power, Fascism, Police, Protest, Movie\end{tabular} \\ \hline
% 13                 & \begin{tabular}[c]{@{}c@{}}Giorgia Meloni, Blessing, God, Greeting,\\ Woman, Friendly,\end{tabular}                      \\ \hline
% 14                 & \begin{tabular}[c]{@{}c@{}}Berlusconi, President, Right-wing, Amnesty, Win, Govern,\\ Home, Citizenship Income, Pay\end{tabular}                      \\ \hline
% \end{tabular}
% \end{table}






% \begin{table}[h]
% \scriptsize
% \caption{IT - General - Example of 5 communities. Put the Italy General here.}
% \begin{tabular}{|c|c|}
% \hline
% \textbf{Community} & \textbf{Key Words}                                                                                                                          \\ \hline
% 1                 & \begin{tabular}[c]{@{}c@{}}Coach, Supporter, League, Goal, Penalty Kick,\\ Season, Field, Jersey\end{tabular}     \\ \hline
% 3                 & \begin{tabular}[c]{@{}c@{}}Choreography, Classical, Phone-in vote,\\ Sacrifice, Improvisation, Support, Love\end{tabular}     \\ \hline
% 9                 & \begin{tabular}[c]{@{}c@{}}Amici, Sing, Talent, Poll, Victory, Merit,\\ Hope, Capable \end{tabular}     \\ \hline
% 16                 & \begin{tabular}[c]{@{}c@{}}Vasco, Rock King, Stadium, Stage,\\ Show, Great, Fly\end{tabular} \\ \hline
% \end{tabular}
% \end{table}

\subsection{Psycholinguist analysis}

In this section, we study the psycholinguistic properties of comments, aiming at finding similarities and differences in the way commenters of communities communicate. We rely on the Linguistic Inquiry and Word Count (LIWC) tool to %highlight the most significant and peculiar attributes \fm{significant and peculiar? not a good description of LIWC}.\footnote{\url{https://liwc.wpengine.com/}}. LIWC is a text analysis tool that
calculate the degree at which various categories of words (called attributes in the LIWC terminology) are used in a text. For each community, we run LIWC on every comment and compute the average frequency of the attributes over the comments.
% Here, we select all comments from each community, and directly run LIWC on each. LIWC returns the percentage of each attribute in each comment. With these, we compute the average over the comments of each community for each attribute.

We then look for statistical differences between communities based on the average values of the attributes as described in Section \ref{sec:methodology}. For Brazil's scenario, we identify 62 attributes (from the 64 available in LIWC's Portuguese dictionary) for which differences across communities  are statistically significant\footnote{We use the non-parametric test of Kruskal to test attributes that have distinct distribution among the communities comments and consider a p-value of 0.01 we discard attributes no significant.}. For Italy, we identify 77 (from 83 available in the LIWC Italian dictionary) 
%\ana{both politics and general scenarios?}. %, albeit there are still an expressive number of attributes with statistical difference between the averages.
From those, we select the 5 (five) attributes that exhibit the largest variability across communities in terms of Gini index. We use them to create visualizations that can better highlight topics associated to communities. 


Figure~\ref{Fig:Liwc_politics} shows heatmaps for the top-5 attributes found for the Brazilian (left) and Italian (right) politics scenarios. The heatmap cells in a column indicate the relative deviation of the given attribute for the given community from the other communities. Locations are color-coded red (resp.\ blue) when the attribute is more (resp.\ less) present than the average. To this end, each column (attribute) is z-score normalized -- i.e.,$z = (x - mean)/std$. Thus, each column value gets subtracted the average of the column, then it is divided by the standard deviation of the column. 
In order to clarify the meaning of each attribute, Table~\ref{Tab:LIWC} includes examples of words belonging to each of them found in LIWC's documentation. %This allows us to better appreciate variations, on the same range.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{fig/Fig15.png}\caption{Top 5 LIWC attributes.}\label{Fig:Liwc_politics}
\end{figure*}

The results in Figure \ref{Fig:Liwc_politics} show that the communities are quite different with respect to the selected attributes. For instance, for the Brazil - politics scenario, communities 6, 10, 3 and 7 frequently use words regarding \emph{death}, but seldom words related to health. Communities 2, 5 and 4 show positive scores on almost all attributes. Community 13 focuses mostly on \emph{health}. In Italy, community 6 is very focused on \emph{religion} (commenters debated Salvini's post that depicts a Rosary). Community 12 and 13 exhibit some hate speech. In summary, LIWC is a useful tool to analyze the content of comments entered by commenters, complementing the TF-IDF analysis with information on the topics being debated. We find that communities debate on different topics and using a different lexicon. 

 
% \ch{Methodology of LIWC Analysis:
% \begin{enumerate}
%     \item First of all, we removed comments with less than 100 characters. If all comments were used, the analysis was very noised. There is no a clear justification to do it, maybe to capture and use only the more elaborated comments. Notice that here, we are considering the original comment. There is no pre-processing carried out on TF-IDF analysis.
    
%     \item Then, we ran the LIWC on the comments getting the percentage of words of a given attribute (Dimension as refered by LIWC) in each comment. Now, we have  for each LIWC attribute, the distribution of the percentage of this attribute in all comments carried out by a given community.

%     \item Then, we did a hypotheses test non-parametric Kruskal to test attributes that have distinct distribution among the communities comments. For a p-value of 0.5 we discard the no significant attribute. Still, a lot of attributes is present, once that the test assumes as hypotheses H0 that at least one distribution is different from the others. We, then, compute Gini Index to get the top 5 attributes with a higher Gini index, which is an indicative of the more variation(difference) between the communities.     
    
%     \item There are plots for Brazil and Italy politics, for the average and confidence interval for the top 5 attributes. 
    
%     \item An important observation is that in Liwc the analysis is done based on the difference relative. For instance, if a community has 2 percent of words related to death and others has 4 percent, based on the confidence interval we can define a significant difference between the two communities and a relative difference. If you to see in the LIWC web site the percentages in general are low for many categories. Maybe, we can put an example of word for each category in order to clarify.  
% \end{enumerate}}



% \textbf{\ch{Hard to explain. There is no a general pattern.}}





\begin{table}[h]
\caption{Example of Words for LIWC Attributes.}
\label{Tab:LIWC}
\begin{tabular}{|c|c|}
\hline
\textbf{Attribute} & \textbf{Example of Words} \\ \hline
Home               & kitchen, landlord         \\ \hline
Family             & daughter, dad, aunt       \\ \hline
Religion           & altar, church, God        \\ \hline
Health             & clinic, flu, pill         \\ \hline
Death              & bury, coffin, kill        \\ \hline
Money              & audit, cash, owe          \\ \hline
We                 & we, us, our               \\ \hline
Profanity          & fuck, damn, shit          \\ \hline
\end{tabular}

\end{table}







% \begin{figure}[!h]
%     \centering
%     \subfloat[PCA BR Politics]{\includegraphics[width=0.33\columnwidth]{fig/journal/PCA_LIWC-BR.pdf}\label{Fig:}}  
%     \subfloat[PCA IT Politics]{\includegraphics[width=0.33\columnwidth]{fig/journal/PCA_LIWC-IT.pdf}\label{Fig:}}  
%     \caption{...}
% \end{figure}

% \begin{figure}[!h]
%     \centering
%     \subfloat[Explainability BR]{\includegraphics[width=0.40\columnwidth]{fig/journal/Explainability_LIWC-BR.pdf}\label{Fig:}}  
%     \subfloat[Explainability IT]{\includegraphics[width=0.40\columnwidth]{fig/journal/Explainability_LIWC-IT.pdf}\label{Fig:}}  
%     \caption{...}
% \end{figure}

% \begin{table}[h]
% \begin{tabular}{|c|c|c|}
% \hline
% \textbf{Symbol} & \textbf{Brazil} & \textbf{Italy} \\ \hline
% A               & Home            & Religion       \\ \hline
% B               & Family          & Money          \\ \hline
% C               & Religion        & We             \\ \hline
% D               & Health          & Profanity      \\ \hline
% E               & Death           & Death          \\ \hline
% \end{tabular}
% \end{table}



==> makefile <==
DOC=Main

all:
	pdflatex $(DOC)
	bibtex   $(DOC)
	pdflatex $(DOC)
	pdflatex $(DOC)

clean:
	find . -name '*~' -exec rm -f {} \;
	find . -name '*.aux' -exec rm -f {} \;
	rm -f texput.log $(DOC).log $(DOC).ps $(DOC).toc $(DOC).lo* $(DOC).bbl $(DOC).blg $(DOC).dvi $(DOC).out $(DOC).synctex.gz diff.bbl diff.blg

zip: ${sources} ${pdffiles}
	rm -f $(DOC).zip && zip -r $(DOC).zip *.tex *.bib *.bbl *.cls fig Makefile makefile

diff:
		latexdiff -c first_version/latexdiff_conf.txt \
				  --preamble=first_version/latexdiff_preamble.tex \
	              --flatten first_version/Main.tex Main.tex > diff.tex
		#pdflatex diff
		#bibtex diff
		pdflatex diff
		pdflatex diff
		
# 


==> temp2.tex <==
\section{Modeling Collective Behavior}\label{sec:rw_collective}


Collective behavior is a wide and complex concept covering different kinds of behaviors, structures, processes in varied contexts. In essence, collective behavior is a multidisciplinary topic of investigation, being studied by researchers in areas such as Sociology, Anthropology, Psychology, Political Science, Economics and, more recently, Computer science \cite{Del:2013}. The concept of collective behavior has changed over time, broadening in response to changes in social relations and to the evolution of society. One of the main reasons was technological advances, which allows collective behavior to reach global scale \cite{Del:2013}. Popularity of online content \cite{Lu:2019-co-drive, Lu:2020, De:2020}, human mobility \cite{Silva:2014, Yang:2016},  market transaction \cite{Peron:2011, Mateo:2019, Saeedian:2019} are notable examples where collective behavior has been studied. According to the American Sociologist Neil Smelser, ``Collective behavior refers to the kinds of \textit{activities} engaged in by \textit{sizable} but \textit{loosely organized groups of people}.'' \cite{Smelser:2011, Collective:2020}. In other words, according to this definition, collective behavior is essentially associated with a considerable number of people acting in a given context in general. Although there may be any small structure for a subset of these people who act collectively, it is extrapolated by the scale of joint actions considering all individuals. Therefore, they still constitute a loosely organized group.

In Computer Science, the modeling of collective behavior has been explored across different frontiers. The combination of new technologies and methodologies enables the crawling, storage and processing of large volumes of data that are sources of information and can contribute to a multidisciplinary sphere. In such a context, distinct computational models have been used to study collective behavior. In the following, we discuss some prior efforts in that direction.

For example, the adoption of models based on time series has allowed studies on how the preference for content generated by influential users favors bursts of engagement on Twitter \cite{De:2020}. In \cite{Mitra:2017}, the authors showed a relationship between the dynamics of news spreading on Twitter and their level of credibility. They observed that news with lower levels of credibility tends to attract more users to spread them. Lehmann et al. \cite{Lehmann:2012} showed that the diffusion of hashtags on Twitter analyzed from a collective perspective is naturally driven by exogenous factors. That is, co-interactions through hashtags posts are mostly expressed by common feelings that instigate users' actions.

In a different direction, prior studies explored machine learning techniques to analyze collective behavior patterns. For example, the authors of \cite{Yang:2016} proposed to extract cultural similarities in cities by analyzing patterns of collective behavior through the use of Location-Based Social Networks data.  Similarly, Silva et al. proposed to map people’s mobility between places using Location-Based Social Networks (LBSN) data to build a transition graph model. Using such model, the authors analyzed patterns of human mobility in different cities, discussing how to identify similarities and differences in human dynamics by grouping cities according to characteristics of people's mobility \cite{Silva:2014}. Other prior studies by the same authors investigated the emergence of gender preference for venues in a given region in the real world \cite{Gender:2017} and user preferences regarding eating and drinking habits across populations at different scales, e.g., countries, cities, or neighborhoods \cite{Silva:2017}. 

Other approaches propose the use of alternative models to analyze collective behavior. As an example, Lu et al. \cite{Lu:2019-co-drive} proposed a \textit{survival model} to identify factors that motivate and drive collective attention under content generated on online social networks. Orthogonally, Martin-Gutierrez et al.~\cite{Martin-Gutierrez:2020} proposed a probabilistic framework to analyze how actions performed by individuals embedded in a social system trigger collective reactions (or responses). In \cite{Gleeson:2014}, the authors propose a generative model to analyze how users collectively interact with Facebook applications taking into account the history of recent decisions and the cumulative popularity of each application.

Focusing on network-oriented models, closer to the goals of this work, a number of studies target the analysis of collective behavior notably in social media applications. For example, Lu et al. \cite{Lu:2020} proposed a framework for modeling collective behavior in cascading social systems (e.g., Twitter and Weibo). The authors found that users following the same profile can be organized into different groups, each one with particular characteristics driving such collective behavior, e.g., timing, structure, posts topic, and user interests. The author of \cite{Liu2018:collectiveFacebook} used the Facebook and Wiki-talk (A dataset build on edits on user talk pages on Wikipedia) aimed at understanding how user's  \textit{social signature} changes over time considering their ego network.  In the same direction, Xu et al.~\cite{Xu:2018} aimed at developing strategies to predict user behavior, given some knowledge of the behavior adopted by the user's neighbors in the network.

By associating users with common interests, Awal et al.~\cite{Awal:2019} examined collective preferences by adopting an overlapping community detection approach. Their goal was  to extract information and predict which categories of articles a user would read or would be interested in reading, based on his/her social collective actions on a consumer review site. Gao et al. modeled human behavior during different extreme events by correlating data from Twitter and GoogleTrends. The goal of the authors was to  assess how human risk and emotional intensity generate collective responses in different regions and how these responses evolve over time. The results of a case study of the  2011 Japanese earthquake show different communities emerging with different perceptions and actions about the event studied \cite{Gao:2016}. Similarly, Kuvsen et al.\cite{Kuvsen:2020} analyzed the communication pattern among groups of users on Twitter in the face of several natural disasters. The authors reveal how the discussions around the observed disasters exhibit a different underlying structure in terms of connectivity (motifs) varying according to the sentiment of messages. In a broader analysis, Zhao et al. \cite{Zhao:2010} examine how motifs representing topological structures of communication in different Online Social Networks. The authors identified different communication patterns and analyzed how frequent and stable they are over time.

In short, there is a large number of studies in different areas but notably in Computer Science, focused on modeling collective behavior. Similar to some of the aforementioned prior efforts, we here also propose a network-oriented approach.  Naturally, the collective actions of groups of individuals constitute what we here refer to as \textit{co-interactions}, which can be modeled by a network. Consequently, this favors the extraction of patterns of different natures (e.g., structural, contextual and temporal). However, most of the previous efforts neglect some aspects of paramount importance that we will discuss and address throughout this paper. In particular, many such co-interactions occur from random and sporadic behavior, thus reflecting very weak relations from the perspective of analyzing collective behavior to understand the target phenomenon. Thus, it is important to filter out  such noise,  focusing only on those network edges that are really relevant (or salient) for the purpose of characterizing collective behavior \cite{Benson2:2018, De:2020, Ghalmane:2020}. 

Similarly, focusing on the extraction of communities of people exhibiting collective behavior, the adoption of community detection approaches seems a natural strategy to identify structural properties of how individuals relate and provide a view of how the system is structured. Moreover, mapping the dynamics of these groups over time converge or contrast is something seldom explored by previous studies, although it  constitutes a fundamental property of any collective behavior \cite{Del:2013, Gleeson:2014, Mitra:2017}. 

Here, our main hypothesis is that considering these previously neglected elements together can provide valuable insights about collective behavior in a given system. This imposes a series of challenges, starting with the possibility of proposing a generalized and agnostic modeling approach. In the following sections, we discuss other prior studies that are also related to this work, including prior techniques employed in the analysis of collective behavior.  We start by discussing prior studies  on modeling user co-interactions, which, though closely related to our current goal, differs by not necessarily aiming at uncovering patterns of collective behavior. 

\section{Modeling User Co-Interactions}\label{sec:rw_modeling_user_co_interactions}   


A plethora of phenomena related to human interactions online and in the real world have been analyzed using concepts from complex networks. Yet, many of these interactions occur among multiple (potentially two or more) entities simultaneously, here referred to as  \textit{co-interactions}. Acknowledging the distinct properties of co-interactions, some recent studies have empirically analyzed them through the lens of \textit{higher-order} models. Such models focus on preserving the different structures of connectivity that can occur as two or more individuals interact with each other \cite{Battiston:2020, Yoon:2020}. 

In the most basic form, these structures are represented by different motifs (e.g., triangular motifs, star, structural hubs, etc) \cite{Benson:2016b, Rossi:2018}. Indeed, Benson et al.~\cite{Benson:2016b} explored the diversity of such co-interactions to analyze how they build networks with diverse structural patterns. Similarly, Rossi et al.~\cite{Rossi:2018} proposed a general framework to learn higher-order structures embedding representations  based on distinct motifs, while others have used neural networks to extract latent patterns from signals to forecast new co-interactions  \cite{Meng:2018, Hu:2019}. Adamic et al.~\cite{Adamic:2008} analyzed how co-interactions take place on Yahoo Answers. The authors found differing kinds of interaction represented by motifs in the question-answer networks that vary according to the topic. 


Here, we focus on the densest and most uniform form of co-interactions, where all individuals interact with each other, a particular type of motif known as clique \cite{Battiston:2020}. For such case, the literature adopts different nomenclatures, including \textit{sets} of interactions, sequences of \textit{associations}, \textit{cliques}, and \textit{multi-actor} interactions \cite{Kumar:2019, Lerner:2019, Battiston:2020, Yoon:2020}. These co-interactions constitute an important substructure for some complex systems, exhibiting diverse properties that are relevant to the study of the (often global) phenomenon of interest \cite{Benson2:2018, Meng:2018}. Examples of such co-interactions are online shopping carts with a set of items being purchased together, co-authors of scientific publications, people co-visiting the same places driven by cultural interests, groups of users commenting or sharing the same topic on a social media application \cite{Yang:2016, Benson:2018, Newman:2018, Nobre:2020, Giglietto:2020, Brito:2020}. 

Moreover, we are interested in looking at how a sequence of such co-interactions, driven by actions of interest of multiple individuals build a network.  To that end, we model them by projecting them into a weighted and undirected graph where nodes (or vertices) correspond to individuals and a weighted edge links two individuals according if they have already interacted. The weight corresponds to the number of interactions both individuals shared in common during the period under analysis.  However, as already argued \cite{Liebig:2016, Benson:2018, Coscia:2019, Cao:2019,  Kumar:2020}, such projected networks may include a large number of random, sporadic and weak edges that are not really part of the fundamental underlying network component representing the target phenomenon. Indeed, although this practice of projecting the original network into a graph of pairwise connections has been widely adopted, little attention has been paid to understanding how the projection considering all co-interactions may obfuscate relevant structural properties in the projected network.

For example, Cruickshank et al. \cite{Cruickshank:2020} proposed to analyze discussion topics on Twitter by modeling a sequence of networks of co-interaction built on co-occurrences of hashtags used by tweet users. Moreover, other information is considered to model the network, for instance, the textual similarity of Tweets using the same hashtag. Then, a community detection method is applied to identify topical clusters of hashtags. In another work, the authors analyzed the online hate of such communities \cite{Uyheng:2021}. Similarly, Pacheco et al. use different features (e.g., similar hashtags, images or chronological events) of users to model co-interactions between them. With that, the authors reveal different patterns that suggest coordinated behavior on Twitter.


More recently, some studies have shown the importance of removing random or weak edges to reveal an underlying structure (i.e., the backbone) in networks formed by co-interactions \cite{Grinberg:2019, Malang:2020, Coscia:2019, Mattsson:2020, Mattsson2:2020, Jaffe:2020, Jiang:2020}. For example, Leão et al. showed how removing random edges in co-authoring networks converge to a topology with more pure social relationships and better quality community structures, compared to the original complete network \cite{Leao2018}. Another example is the study of information dissemination on the WhatsApp platform \cite{Nobre:2020}, where the authors explored a network of co-sharing patterns (i.e., a network connecting users who shared the same piece of content) to reveal important properties of information spread on the platform. 


Thus, as part of our approach to model co-interactions, we must tackle the challenges of using the projected network in a very rich but dynamic environment, notably the presence of a potentially large number of weak and possibly irrelevant edges in online social applications. Unlike of the prior works, we investigate strategies that remove such noise and reveal edges in our co-commenters network that, in fact, contribute to the study of information dissemination from the co-interaction of users on Instagram.  Moreover, we  investigate strategies to extract the backbone in such context and discuss their limitations in the next section. 


==> temp_.tex <==
With no specific focus on political debates, other studies have also analyzed user engagement from different perspectives. For example, Kang et al.~\cite{Kang:2020} studied a well-known strategy to trigger user interactions in social media, namely mentioning a friend in a comment. The authors proposed a model capable of classifying mentions into three categories based on its motivation:  information-oriented,  relationship-oriented, and  discussion-oriented. Results: This paper investigates the current practice of user tagging in Instagram by collecting a large-scale data that includes 9 K posts and their 4 M comments shared by 3 M users. Our analysis reveals that 54.8\% of the comments contain user tagging, meaning that user tagging is widely-used in Instagram. To shed light on why Instagram users tag friends in comments, we develop a learning-based model that classifies the motivation of user tagging into one of the following motivations: (i) information-oriented, (ii) relationship-oriented, and (iii) discussion-oriented. We then apply our model to the comments with user tagging in our data, and reveal that user tagging is often used for interpersonal communication with friends. \textbf{Our position:} We found that engagement through these mechanisms varies according to the topic, notably, in politics we see much more frequent use not only of tagging, but also of XXX hashtags, analyze FIGURE 8.


Jaakonmäki et al.~\cite{Jaakonm:2017} analyzed the influence of the content posted for social media marketing. They used machine learning algorithms to extract textual and visual content features from  posts, along with creator and context features, to  model their influence on user engagement. 

\textbf{Results:} Our results indicate that choosing the right influencer affects user engagement, as the creator related factors—especially the number of followers and the creator’s age and gender—play the most significant role among all predictors. Similarly, there are certain days and hours (i.e., contexts) during which the audience is more likely to be engaged than at others. Influencer marketing professionals can use this information to choose bloggers and define the launch time of social media marketing campaigns. Our findings regarding content features can also guide content-creation strategies for social media marketing, thereby responding to marketers’ need to improve their understanding of what types of content are the most engaging [1], [36]. For example, our results suggest that pictures with people and scenery and emojis that express positive emotions (e.g., relief, love, joy) increase engagement. An open issue to be explored in future work concerns the consequences of designing content according to this knowledge. For example, it is possible that, as professional bloggers and marketers increase their use of content that is predicted to be highly engaging, the content will lose effectiveness: If everybody posts pictures with women in front of nature scenes on Friday evenings at 8:00 p.m., a kind of fatigue effect may set in. However, the approach we presented here can easily be repeated with minimal costs in order to monitor such developments in near real time.

\textbf{Our position:}  We found evidence of key elements for a post to attract a large number of users (represented here by communities). In addition, we also reveal that different communities are formed by different subsets of posts under the same influence. This occurs mainly in politics, indicating that the political mechanisms of communication can be much more assertive in terms of content and audience.


In another direction, Yang et al.~\cite{Yang:2019} studied the brand mentioning practices of influencers, finding that audience has highly similar reactions to sponsored and non-sponsored posts. They also proposed a neural network model to classify the sponsorship of posts combining network embedding  with features related to the posts and followers. Similarly, 
Kim et al. \cite{Kim:2020} proposed a multimodal deep learning model that uses contextual information of posts, including textual and image content,  to classify influencers as well as their posts into specific topics, such as, food, fashion and traveling. 

Other studies have analyzed properties of the textual content shared by Instagram users. For example, Zhan et al.~\cite{Zhan:2018} analyzed the sentiment of captions of Instagram posts to provide a preview of the content to the reader. Arslan et al.~\cite{Arslan:2019} also used sentiment analysis tools to develop a message-level emotion  classifier, with the goal of detecting cyberbullying. With a similar goal, Gupta et al.~\cite{Gupta:2020} focused on the temporal perspective, showing that, cyberbullying activities exhibit recurrent temporal patterns such as the occurrence of bursts. In the same direction, Kao et al.~\cite{Kao:2019} proposed a social role detection framework  to analyze cyberbullying on online social platforms, taking Instagram as one of their case studies. The framework considers the roles of victim, bully and supporter, which are automatically identified by analyzing comment network and linguistic properties.

